Quantized mixed tensor space and Schur-Weyl duality

Let $R$ be a commutative ring with one and $q$ an invertible element of $R$. The (specialized) quantum group ${\mathbf U} = U_q(\mathfrak{gl}_n)$ over $R$ of the general linear group acts on mixed tensor space $V^{\otimes r}\otimes {V^*}^{\otimes s}$ where $V$ denotes the natural $\mathbf U$-module $R^n$, $r,s$ are nonnegative integers and $V^*$ is the dual $\mathbf U$-module to $V$. The image of $\mathbf U$ in $\mathrm{End}_R(V^{\otimes r}\otimes {V^*}^{\otimes s})$ is called the rational $q$-Schur algebra $S_{q}(n;r,s)$. We construct a bideterminant basis of $S_{q}(n;r,s)$. There is an action of a $q$-deformation $\mathfrak{B}_{r,s}^n(q)$ of the walled Brauer algebra on mixed tensor space centralizing the action of $\mathbf U$. We show that $\mathrm{End}_{\mathfrak{B}_{r,s}^n(q)}(V^{\otimes r}\otimes {V^*}^{\otimes s})=S_{q}(n;r,s)$. By \cite{dipperdotystoll} the image of $\mathfrak{B}_{r,s}^n(q)$ in $\mathrm{End}_R(V^{\otimes r}\otimes {V^*}^{\otimes s})$ is $\mathrm{End}_{\mathbf U}(V^{\otimes r}\otimes {V^*}^{\otimes s})$. Thus mixed tensor space as $\mathbf U$-$\mathfrak{B}_{r,s}^n(q)$-bimodule satisfies Schur-Weyl duality.

==> anrs.tex <==
\section{Mixed tensor space as a submodule}\label{section:submodule}

Recall that $\mathbf{U}'$ is the subalgebra of $\mathbf{U}$
corresponding to the Lie algebra $\mathfrak{sl}_n$.

\begin{thm}
  If $m$ is a nonnegative integer, let $\rho_{\mathrm{ord}}:\mathbf U\to
  \mathrm{End}_R(V^{\otimes m})$ be the representation of $\mathbf U$
  on $V^{\otimes m}$. Then 
  \[
  \rho_{\mathrm{ord}}(\mathbf U)=\rho_{\mathrm{ord}}(\mathbf U').
  \]
\end{thm}


 \begin{proof}
%   At the moment, we will only show the first part of the
%   proposition. It is used to show the second part in
%   Theorem~\ref{thm:schurweyl2}.
   Define the \emph{weight} of $\mathbf i\in I(n,m)$ to be
   $\mathrm{wt}(\mathbf i)=\lambda
   =(\lambda_1,\ldots,\lambda_n)$, such that
   $\lambda_i$ is the number of entries in 
   $\mathbf i$, that are equal to
   $i$.
   If $\lambda=(\lambda_1,\ldots,\lambda_n)$ is a composition of $m$ into
   $n$ parts, i.~e.~ $\lambda_1+\ldots+\lambda_n=m$,
   let $V^{\otimes m}_\lambda$ be the $R$-submodule of
   $V^{\otimes m}$ generated by all $v_{\mathbf  i}$ with 
   $\mathrm{wt}(\mathbf i)=\lambda$. Then $V^{\otimes m}$ is the direct
   sum of all $V^{\otimes m}_\lambda$, where $\lambda$ runs through the
   set of compositions of $m$ into $n$ parts. Let $\varphi_\lambda$ be the
   projection onto  $V^{\otimes m}_\lambda$.
   \cite{green} shows, that the restriction of 
   $\rho_{\mathrm{ord}}:\mathbf U\to
   S_q(n,m)$ to any subalgebra $\mathbf U'\subseteq \mathbf U$ 
   is surjective, if
   the subalgebra $\mathbf U'$ contains
   the divided powers $e_i^{(l)},f_i^{(l)}$
   and preimages of the projections $\varphi_\lambda$. 

   Therefore, we define a partial order on
   the set of compositions of $m$ into $n$ parts by 
   $\lambda\preceq\mu$ if and only if 
   $(\lambda_1-\lambda_2,\lambda_2-\lambda_3,\ldots,
   \lambda_{n-1}-\lambda_n)\leq(\mu_1-\mu_2,\mu_2-\mu_3,\ldots,
   \mu_{n-1}-\mu_n)$ in the lexicographical order. 
   It suffices to show, that for each composition
   $\lambda$, there exists an element $u\in {\mathbf U}'$ such that
   $uv_{\mathbf i}=0$ whenever $\mathrm{wt}(\mathbf i)\prec \lambda$ (i.~e.~
   $\mathrm{wt}(\mathbf i)\preceq \lambda$ and 
   $\mathrm{wt}(\mathbf i)\neq \lambda$) and 
   $uv_{\mathbf i}=v_{\mathbf i}$ whenever $\mathrm{wt}(\mathbf i)=
   \lambda$. 
   In Theorem~4.5 of \cite{lusztig}, it
   is shown that certain elements 
   \[ \left[\genfrac{}{}{0pt}{}{K_i;c}{t}\right]
   :=\prod_{s=1}^t
   \frac{K_iq^{c-s+1}-K_i^{-1}q^{-c+s-1} }{q^s-q^{-s}}
   \]
   are elements of ${\mathbf U}'$ for $i=1,\ldots,n-1,c\in\mathbb{Z}$ and
   $t\in\mathbb{N}$. 
   Let 
   \[u:=\prod_{i=1}^{n-1} 
   \left[\genfrac{}{}{0pt}{}
     {K_i;m+1}{\lambda_i-\lambda_{i+1}+m+1}
   \right],
   \] 
   which is an element of ${\mathbf U}'$ since 
   $\lambda_i-\lambda_{i+1}+m+1>0$. 
   Then $u$ has the desired properties. 
 \end{proof}
% %  For the moment, let $R=\mathbb{Z}[q,q^{-1}]$ and
% %  $Q=\mathbb{Q}(q)$. Then  ${\mathbf U}_R'$ is a subalgebra
% %  of $\mathbf U_Q$.
% %  In Theorem~4.5 of \cite{lusztig}, it
% %  is shown that certain elements 
% %  \[ \left[\genfrac{}{}{0pt}{}{K_i;c}{t}\right]
% %  :=\prod_{s=1}^t
% %   \frac{K_iq^{c-s+1}-K_i^{-1}q^{-c+s-1} }{q^s-q^{-s}}
% %   \]
% %   are elements of ${\mathbf U}_R'$ for $i=1,\ldots,n-1,c\in\mathbb{Z}$ and
% %   $t\in\mathbb{N}$. 
% %   Define the \emph{weight} of $\mathbf i\in I(n,m)$ as
% %   $\mathrm{wt}(\mathbf i)=\alpha
% %   =(\alpha_1,\ldots,\alpha_n)$, such that
% %   $\alpha_i$ is the number of entries in 
% %   $\mathbf i$, that are equal to
% %   $i$. Then 
% %   \begin{eqnarray*}
% %     \left[\genfrac{}{}{0pt}{}{K_i;c}{t}\right]v_{\mathbf i}%&=&
% %     % \prod_{s=1}^t
% %     % \frac{q^{\alpha_i-\alpha_{i+1}+c-s+1}-
% %     %   q^{-\alpha_i+\alpha_{i+1}-c+s-1} }
% %     % {q^s-q^{-s}}v_{\mathbf i}=
% %     % \begin{bmatrix}\alpha_i-\alpha_{i+1}+c\\t\end{bmatrix}_qv_{\mathbf
% %     %   i}\\
% %     &=&\begin{cases}
% %       v_{\mathbf i}&\text{ if }\alpha_i-\alpha_{i+1}+c=t\\
% %       0&\text{ if }\alpha_i-\alpha_{i+1}+c\in\{0,\ldots,t-1\}.
% %     \end{cases}
% %   \end{eqnarray*}
% %   If $R$ is an arbitrary commutative ring with $1$, these elements are
% %   still defined and the formulas are
% %   still valid.

% %   If $\lambda=(\lambda_1,\ldots,\lambda_n)$ is a composition of $m$ into
% %   $n$ parts, i.~e.~ $\lambda_1+\ldots+\lambda_n=m$,
% %   let $V^{\otimes m}_\lambda$ be the $R$-submodule of
% %   $V^{\otimes m}$ generated by all $v_{\mathbf  i}$ with 
% %   $\mathrm{wt}(\mathbf i)=\lambda$. Then $V^{\otimes m}$ is the direct
% %   sum of all $V^{\otimes m}_\lambda$, where $\lambda$ runs through the
% %   set of compositions of $m$ into $n$ parts. Let $\varphi_\lambda$ be the
% %   projection onto  $V^{\otimes m}_\lambda$. We claim, that for each
% %   $\lambda$ there exists an element of ${\mathbf U}'$ such that
% %   $uv=\varphi_\lambda v$
% %   for all $v\in V^{\otimes m}$. Therefor, we define a partial order on
% %   the set of compositions of $m$ into $n$ parts by 
% %   $\lambda\preceq\mu$ if and only if 
% %   $(\lambda_1-\lambda_2,\lambda_2-\lambda_3,\ldots,
% %   \lambda_{n-1}-\lambda_n)\leq(\mu_1-\mu_2,\mu_2-\mu_3,\ldots,
% %   \mu_{n-1}-\mu_n)$ in the lexicographical order. It is obvious that
% %   this relation is reflexive and transitive. Suppose that $\lambda
% %   \preceq \mu$ and $\mu\preceq\lambda$. Then
% %   $\mu_i-\mu_{i+1}=\lambda_i-\lambda_{i+1}$ for $i=1,\ldots,n-1$. Thus 
% %   $\lambda_1+\lambda_2+\ldots +\lambda_n-n\lambda_n=
% %   \sum_{i=1}^{n-1}i(\lambda_i-\lambda_{i+1})=
% %   \sum_{i=1}^{n-1}i(\mu_i-\mu_{i+1})=
% %   \mu_1+\mu_2+\ldots +\mu_n-n\mu_n $. Since
% %   $\sum_{i=1}^n\lambda_i=m=\sum_{i=1}^n\mu_i$, we have $\lambda_n=\mu_n$
% %   and thus $\lambda=\mu$. This shows that the relation is
% %   antisymmetric. Thus it suffices to show, that for each composition
% %   $\lambda$, there exists an element $u\in {\mathbf U}'$ such that
% %   $uv_{\mathbf
% %     i}=0$ whenever $\mathrm{wt}(\mathbf i)\prec \lambda$ (i.~e.~
% %   $\mathrm{wt}(\mathbf i)\preceq \lambda$ and 
% %   $\mathrm{wt}(\mathbf i)\neq \lambda$) and 
% %   $uv_{\mathbf i}=v_{\mathbf i}$ whenever $\mathrm{wt}(\mathbf i)=
% %   \lambda$. 
% %   Let 
% %   \[u:=\prod_{i=1}^n 
% %   \left[\genfrac{}{}{0pt}{}
% %     {K_i;m+1}{\lambda_i-\lambda_{i+1}+m+1}
% %   \right],
% %   \] 
% %   which is an element of ${\mathbf U}'$ since 
% %   $\lambda_i-\lambda_{i+1}+m+1>0$. 
% %   If  $\mu = \mathrm{wt}(\mathbf i)$, then 
% %   \[
% %   uv_{\mathbf i}=\prod_{i=1}^n 
% %   \left[\genfrac{}{}{0pt}{}
% %     {\mu_i-\mu_{i+1}+m+1}{\lambda_i-\lambda_{i+1}+m+1}
% %   \right]_qv_{\mathbf i}
% %   \]
% %   For $\mu=\lambda$ this is equal to $v_{\mathbf i}$. 
% %   If $\mu\prec \lambda$, then there is some $k$ such that
% %   $\mu_k-\mu_{k+1}< \lambda_k-\lambda_{k+1}$. Then
% %   $\mu_k-\mu_{k+1}+m+1\in \{0,\ldots,\lambda_i-\lambda_{i+1}+m\}$, and
% %   we have $uv_{\mathbf i}=0$. 


% %   In    {\cite[Corollary~3.7]{green}},
% %   it is shown that for $R=\mathbb{Z}[q,q^{-1}],Q=\mathbb{Q}(q)$, 
% %   the homomorphism
% %   $\mathbf U_Q\to S_q(n,m)$ is surjective. The preimages of basis elements 
% %   of the $q$-Schur algebra are explicitly given and lie
% %   in the $R$-subalgebra $\tilde{\mathbf U}$ of $\mathbf U_Q$ generated by 
% %   $e_i^{(l)},f_i^{(l)}$ and certain elements 
% %   $\left[\genfrac{}{}{0pt}{}{q^{h_i};0}{t}\right]\in \mathbf U_Q$. 
% %   The proof shows that
% %   the restriction of 
% %   this  homorphism  to any $R$-subalgebra, which contains the
% %   elements $e_i^{(l)},f_i^{(l)}$ and elements that map to the
% %   $\varphi_\lambda$, is also surjective. (The projections
% %   $\varphi_\lambda$ correspond to diagonal matrices $[D]$ in \cite{green}.) 
% %   We have just shown that ${\mathbf U}'$ contains such elements, thus
% %   ${\mathbf U}'\subseteq {\mathbf U}\subseteq \tilde{\mathbf U}$
% %   all map to the same image. 
% %   The same now holds for any commutative ring $R$ with $1$. \qed







% It is well known, that the action of $\mathbf U$ and thus the action
% of 
% $\mathbf U'$ on ordinary tensor space generates all of
% $\mathrm{End}_{\mathcal{H}_m}(V^{\otimes m})$ where $\mathcal{H}_m$
% is the Hecke algebra of type $A$, see for example \cite{green}.
% We will need this result for $m=r+(n-1)s$.
% \begin{thm}
%   Let $S_q(n,m)$ be the $q$-Schur algebra introduced in
%   \cite{dipperjamesschur} as the algebra of
%   $\mathcal{H}_m$-endomorphisms of $V^{\otimes m}$. Then 
%   \[ 
%   \rho_{\mathrm{ord}}(\mathbf U)=\rho_{\mathrm{ord}}(\mathbf U')=S_q(n,m)
%   \]
% \end{thm}
The next lemma is motivated by \cite[\S6.3]{dipperdoty}.
\begin{lem}\label{lem:monomorphism}
  There is a well defined ${\mathbf U}'$-monomorphism 
  $\kappa:{V^*}\to
  V^{\otimes n-1}$
  given by 
  \begin{eqnarray*}
    v_i^*&\mapsto& (-q)^i\sum_{w\in\mathfrak{S}_{n-1}}
    (-q)^{l(w)}v_{(12\ldots\hat{i}\ldots n).w}\\
    &=&(-q)^i\sum_{w\in\mathfrak{S}_{n-1}}
    (-q)^{l(w)}v_{(12\ldots\hat{i}\ldots n)}T_w
    =(-q)^i v_{(12\ldots\hat{i}\ldots n)}
    \sum_{w\in\mathfrak{S}_{n-1}}
    (-q)^{l(w)}T_w
  \end{eqnarray*}
  where $\hat{i}$ means
  leaving out $i$.
%, the symmetric group $\mathfrak{S}_{n-1}$ 
%    acts on $I(n,n-1)$ by place permutation, and
%    $T_w=T_{i_1}T_{i_2}\ldots T_{i_l}\in\mathcal{H}_{n-1}$
%    if $w=s_{i_1}s_{i_2}\ldots
%    s_{i_l}$ is a reduced expression.  
\end{lem}

\begin{proof}
  It is clear, that $\kappa$ is a monomorphism of $R$-modules. 
  By definition, $K_iv_j^*=q^{\delta_{i+1,j}-\delta_{i,j}}v_j^*$ and
  $K_i v_{(1\ldots\hat{j}\ldots n)}=
  q^{1-\delta_{i,j}}q^{\delta_{i+1,j}-1}v_{(1\ldots  \hat{j}\ldots n)}$.
  Thus $\kappa$ commutes with 
  $K_i$. 
  Now $e_iv_j^*=-\delta_{i,j}q^{-1}v_{j+1}^*$. If $j\neq i,i+1$ then 
  \begin{eqnarray*}
    e_i\kappa(v_j^*)&=&
    (-q)^je_i\sum_w(-q)^{l(w)}v_{(1\ldots i i+1\ldots \hat{j}\ldots n)}T_w\\
    &=&-(-q)^j\sum_w(-q)^{l(w)}v_{(1\ldots i i\ldots \hat{j}\ldots
      n)}T_w =0=\kappa(e_iv_j^*)
  \end{eqnarray*}
  For $j=i$ resp.~$i+1$ we get
  \begin{eqnarray*}
   e_i\kappa(v_{i+1}^*)&=&
   (-q)^{i+1}\sum_w(-q)^{l(w)}(e_iv_{(1\ldots  \widehat{i+1}\ldots n)})T_w=0\\
   e_i\kappa(v_i^*)&=&
   (-q)^i\sum_w(-q)^{l(w)}(e_iv_{(1\ldots  \hat{i}i+1\ldots n)})T_w\\
   &=&
    (-q)^{i}\sum_w(-q)^{l(w)}v_{(1\ldots  i \,\widehat{i+1}\ldots n)}T_w
    =-q^{-1}\kappa(v_{i+1}^*)
  \end{eqnarray*}
Furthermore, for $l\geq 2$ we clearly have $e_i^{(l)}v_j^*=0$ and 
$e_i^{(l)}\kappa(v_j^*)=0$. 
The argument for $f_i$ works similarly.  
\end{proof}
Lemma~\ref{lem:monomorphism} enables us to consider the mixed tensor
space $V^{\otimes r}\otimes {V^*}^{\otimes s}$
as a ${\mathbf U}'$-submodule $T^{r,s}$ of
$V^{\otimes r+(n-1)s}$ via an embedding which we will also denote by
$\kappa$.
Thus $\mathfrak{B}_{r,s}^n(q)$ acts on $T^{r,s}$. 

If we restrict the action of
an element of ${\mathbf U}'$ on $V^{\otimes r+(n-1)s}$
or equivalently of the 
$q$-Schur algebra $S_q(n,r+(n-1)s)$
to $T^{r,s}$, then we get an element of 
$\mathrm{End}_R(T^{r,s})$. Since the actions of ${\mathbf U}'$ and
$\mathfrak{B}_{r,s}^n(q)$ commute, this is also an element of 
$\mathrm{End}_{\mathfrak{B}_{r,s}^n(q)}(T^{r,s})$. 
Let $S_q(n;r,s):=\mathrm{End}_{\mathfrak{B}_{r,s}^n(q)}(V^{\otimes r}\otimes
{V^*}^{\otimes s})$, thus we have an algebra homomorphism
$\pi:S_q(n,r+(n-1)s)\to S_q(n;r,s)$ by restriction of the action to
$T^{r,s}\cong V^{\otimes r}\otimes
{V^*}^{\otimes s}$. Our aim is to show that $\pi$ is
surjective, for then each element of
$\mathrm{End}_{\mathfrak{B}_{r,s}^n(q)}(V^{\otimes r}\otimes 
{V^*}^{\otimes s})$ is given by the action of an element of ${\mathbf U}'$. 

\begin{lem}\label{lem:construction}
  Let $M$ be a free $R$-module with basis
  $\mathcal{B}=\{b_1,\ldots,b_l\}$ and let
  $U$ be a submodule of $M$ given by a set of linear equations on the
  coefficients with respect to the basis
  $\mathcal{B}$, i.~e.~there are elements $a_{ij}\in R$ such that 
  $U=\{\sum c_ib_i\in M:\sum_j a_{ij}c_j=0 \text{ for all }i\}$.
  Let $\{b_1^*,\ldots,b_l^*\}$ be the basis of $M^*=\mathrm{Hom}_R(M,R)$ dual
  to $\mathcal{B}$ and let
  $X$ be the submodule generated by all $\sum_j a_{ij}b_j^*$. Then
  $U\cong \left(M^*/X\right)^*$.
\end{lem}
\begin{proof}
    $\left(M^*/X\right)^*$ is isomorphic to the submodule of $M^{**}$
    given by linear forms on $M^*$ that vanish on $X$. Via the natural
    isomorphism $M^{**}\cong M$, this is isomorphic to the set of
    elements of $M$ that are annihilated by $X$. An element $m=\sum_k
    c_kb_k$ is annihilated by $X$ if and only if $0=\sum_{j,k}
    a_{ij}b_j^*(c_kb_k)= \sum_k a_{ik}c_k$ for all $i$ 
    and this is true if and
    only if $m\in U$.
\end{proof}

Note that an element $\tilde\varphi\in (M^*/X)^*$ corresponds to the
element $\varphi=\sum_i \tilde\varphi(b_i^*+X)b_i$ of $U$.  In our
case $S_q(n,m)$ and $S_q(n;r,s)$ are $R$-submodules of $R$-free
algebras, namely $\mathrm{End}_R(V^{\otimes m})$ and
$\mathrm{End}_R(V^{\otimes r}\otimes {V^*}^{\otimes s})$ resp., given
by a set of linear equations, which we will determine more precisely
in Sections \ref{sec:Aqnm} and \ref{sec:Aqnrs}.

\begin{defn}
  Let $A_q(n,m)=M^*/X$ as in Lemma~\ref{lem:construction} where
  $M=\mathrm{End}_R(V^{\otimes m})$ and $U=S_q(n,m)$
  and similarly let $A_q(n;r,s) =M^*/X$ with
  $M=\mathrm{End}_R(V^{\otimes r}\otimes {V^*}^{\otimes s})$ and
  $U=S_q(n;r,s)$. 
\end{defn}
Note that these definitions make sense, since $S_q(n,m)$ and
$S_q(n;r,s)$ are defined as algebras of endomorphisms commuting with
certain endomorphisms, and thus are given by a system of linear
equations. Furthermore,  by Lemma~\ref{lem:construction} we have 
$A_q(n,m)^*= S_q(n,m)$ and $A_q(n;r,s)^*=S_q(n;r,s)^*$.





We will proceed as follows: We will take $m = r+(n-1)s$ and define an
$R$-homomorphism $\iota:A_q(n;r,s)\to A_q(n,r+(n-1)s)$ such that
$\iota^*=\pi: S_q(n,r+(n-1)s)\to S_q(n;r,s)$.  Then we will define an
$R$-homomorphism $\phi:A_q(n,r+(n-1)s)\to A_q(n;r,s)$ such that
$\phi\circ\iota=\mathrm{id}_{A_q(n;r,s)}$ by giving suitable bases for
$A_q(n,r+(n-1)s)$ and $A_q(n;r,s)$. Dualizing this equation, we get
$\pi\circ\phi^*=\iota^*\circ\phi^*=\mathrm{id}_{S_q(n;r,s)}$, and this
shows that $\pi$ is surjective.  Actually $A_q(n,r+(n-1)s)$ and
$A_q(n;r,s)$ are coalgebras and $\iota$ is a morphism of coalgebras,
but we do not need this for our results.



\section{$A_q(n,m)$} \label{sec:Aqnm}

The description of $A_q(n,m)$ is well known, see
e.~g.~\cite{dipperdonkin}.
Let $A_q(n)$ be the free $R$-algebra on
generators $x_{ij}$ ($1\leq i,j\leq n$) subject to the relations
\begin{eqnarray*}
  x_{ik}x_{jk}&=&qx_{jk} x_{ik} \quad\text{ if } i<j\\
  x_{ki}x_{kj}&=&qx_{kj} x_{ki} \quad\text{ if } i<j\\
  x_{ij}x_{kl}&=&x_{kl}x_{ij} \quad\text{ if } i<k \text{ and } j>l\\
  x_{ij}x_{kl}&=&x_{kl}x_{ij}+(q-q^{-1})x_{il}x_{kj}\quad\text{ if } i<k 
   \text{ and }j<l. 
\end{eqnarray*}
Note that these relations define the commutative algebra in $n^2$
commuting intederminates $x_{ij}$ in case $q=1$.
The free algebra on the generators $x_{ij}$ is obviously graded (with
all the generators in degree 1), and since the relations are
homogeneous, this induces a grading on $A_q(n)$. Then
\begin{lem}[\cite{dipperdonkin}]
  $A_q(n,m)$ is the $R$-submodule of $A_q(n)$ of elements of
  homogeneous degree $m$. 
\end{lem}
\begin{proof}
  Since our relations of the Hecke algebra differ from those in 
  \cite{dipperdonkin} ($(T_i-q)(T_i+1)=0$ is replaced by
  $(T_i+q)(T_i-q^{-1})=0$), and thus $A_q(n,m)$ differs as well, we
  include a proof here. 

  Suppose that $\varphi$ is an endomorphism commuting with the action of
  a generator $S_i$. For convenience, we assume that $m=2$ and
  $S=S_1$.
  $\varphi$
  can be written as a linear combination of the basis elements
  $E_{(ij),(kl)}$ mapping $v_k\otimes v_l$ to $v_i\otimes v_j$, and
  all other basis elements to $0$. For the coefficient of
  $E_{(ij),(kl)}$, we write $c_{ik}c_{jl}$, such that
  $\varphi=\sum_{i,j,k,l}c_{ik}c_{jl}E_{(ij),(kl)}$. On the one side
  we have
  \begin{align*}
    S(\varphi(v_k\otimes v_l))&=
    S\left(\sum_{i,j}c_{ik}c_{jl}v_i\otimes v_j\right)\\
    &=\sum_{i<j}c_{ik}c_{jl}v_j\otimes v_i
    +q^{-1}\sum_i c_{ik}c_{il}v_i\otimes v_i
    +\sum_{i>j}c_{ik}c_{jl}(v_j\otimes v_i+(q^{-1}-q)v_i\otimes v_j\\
    &=\sum_{i\neq j}c_{ik}c_{jl}v_j\otimes v_i
    +q^{-1}\sum_i c_{ik}c_{il}v_i\otimes v_i
    +(q^{-1}-q)\sum_{i<j}c_{jk}c_{il}v_j\otimes v_i\\
  \end{align*}

  Now, suppose that $k>l$. Then 
 \begin{align*}
    \varphi(S(v_k\otimes v_l))&=
    \varphi(v_l\otimes v_k+(q^{-1}-q)v_k\otimes v_l)\\
    &= \sum_{i,j}\left(
      c_{jl}c_{ik}+(q^{-1}-q) c_{jk}c_{il}\right)v_j\otimes v_i
  \end{align*}
  Similar formulas hold for $k=l$ and $k<l$.  
  Comparing coefficients leads to the relations given above. 
\end{proof}
$A_q(n,m)$ has a basis consisting of monomials, but it will
turn out to be more convenient for our purposes to work with a
basis of standard bideterminants (see \cite{huangzhang}). Note that
the supersymmetric quantum letterplace 
algebra in \cite{huangzhang} for
$L^-=P^-=\{1,\ldots,n\}, L^+=P^+=\emptyset$ is isomorphic 
to $A_{q^{-1}}(n)\cong A_q(n)^{\mathrm{opp}}$, and we will adjust the
results  to our situation. 

A \emph{partition} $\lambda$ of $m$ is a sequence
$\lambda=(\lambda_1,\lambda_2,\ldots, \lambda_k)$ of nonnegative
integers such that $\lambda_1\geq \lambda_2\geq \ldots \geq
\lambda_k$ and  $\sum_{i=1}^k\lambda_i=m$. Denote the set of
partitions of $m$ by $\Lambda^+(m)$. 
The \emph{Young diagram} $[\lambda]$ 
of a partition $\lambda$ is $\{(i,j)\in
\mathbb{N}\times \mathbb{N}:1\leq i\leq k,1\leq j\leq
\lambda_i\}$. It can be represented by an
array of boxes, $\lambda_1$ boxes in the first row, $\lambda_2$ boxes
in the second row, etc.

A \emph{$\lambda$-tableau} $\mathfrak{t}$ 
is a map  $f:[\lambda]\to \{1,\ldots,n\}$. A
tableau can be represented by writing  the entry $f(i,j)$ into the
$(i,j)$-th box. A tableau $\mathfrak{t}$ is called \emph{standard},
if the entries
in each row are strictly increasing from left to right,
and the entries in each column are nondecreasing downward. In the
literature, this property is also called semi-standard, and the role
of rows and
columns may be interchanged. A pair 
$[\mathfrak{t},\mathfrak{t}']$ of $\lambda$-tableaux is
called a \emph{bitableau}. It is standard 
if both $\mathfrak{t}$ and $\mathfrak{t}'$ are
standard $\lambda$-tableaux. 


Note that the next definition differs from
the definition in \cite{huangzhang} by a sign. 
 \begin{defn}
   Let  $i_1,\ldots ,i_k,j_1,\ldots,j_k$ be  elements of $\{1,\ldots,n\}$,
   For $i_1<i_2<\ldots<i_k$ 
   let the \emph{right quantum minor} be defined by
   \[
   (i_1i_2\ldots i_k|j_1j_2\ldots j_k)_r:=
   \sum_{w\in\mathfrak{S}_k}(-q)^{l(w)}
   x_{i_{w1}j_{1}}x_{i_{w2}j_{2}}\ldots x_{i_{wk}j_{k}}.
   \]
   For arbitrary  $i_1,\ldots ,i_k$, the right 
   quantum minor is then defined by the rule 
   \[ (i_1\ldots i_li_{l+1}\ldots i_k|j_1j_2\ldots j_k)_r:=
   -q^{-1}(i_1\ldots i_{l-1}i_{l+1}i_li_{l+2}
   \ldots i_k|j_1j_2\ldots j_k)_r\]
   for $i_l>i_{l+1}$. 
   Similarly, let the \emph{left quantum minor} be defined by 
   \begin{eqnarray*}
     (i_1\ldots i_k|j_1\ldots j_k)_l&:=& 
     \sum_{w\in\mathfrak{S}_k}(-q)^{l(w)}
     x_{i_1,j_{w1}}x_{i_2j_{w2}}\ldots x_{i_kj_{wk}}
     \text{ if }j_1<\ldots<j_k,\\
     (i_1\ldots i_k|j_1\ldots j_k)_l&:=&-q^{-1} 
     (i_1\ldots i_k|j_1\ldots j_{l+1}j_l\ldots j_k)_l
     \text{ if }j_l>j_{l+1}.
   \end{eqnarray*}
   Finally let  the 
   \emph{quantum determinant} be defined by
   \[{\det}_q:=(12\ldots n|12\ldots n)_r
   =(12\ldots n|12\ldots n)_l.\]
   If $[\mathfrak{t},\mathfrak{t}']$ is a bitableau,
   and $\mathfrak{t}_1,\mathfrak{t}_2,\ldots,\mathfrak{t}_k$  
   resp.~ $\mathfrak{t}_1',\mathfrak{t}_2',\ldots,\mathfrak{t}_k'$ are
   the rows of $\mathfrak{t}$ resp.~$\mathfrak{t}'$, then let
   \[
   (\mathfrak{t}|\mathfrak{t}'):=
   (\mathfrak{t}_k|\mathfrak{t}_k')_r\ldots 
   (\mathfrak{t}_2|\mathfrak{t}_2')_r
   (\mathfrak{t}_1|\mathfrak{t}_1')_r.
   \]
   $(\mathfrak{t}|\mathfrak{t}')$ is called a \emph{bideterminant}.
\end{defn}

\begin{rem}\label{rem:properties}
  We note the following properties of  quantum minors:
\begin{enumerate}
\item 
\begin{eqnarray*}
  (i_1\ldots i_k|j_1\ldots j_k)_r&=&
  -q (i_1\ldots i_k|j_1\ldots j_{l+1}j_l\ldots j_k)_r
  \text{ for }j_l>j_{l+1}\\ 
  (i_1\ldots i_k|j_1\ldots j_k)_l&=&
  -q(i_1\ldots i_{l+1}i_l\ldots i_k|j_1\ldots j_k)_l
  \text{ for }i_l>i_{l+1}.
\end{eqnarray*}


\item If
  $i_1<i_2<\ldots<i_k$ and $j_1<j_2<\ldots<j_k$, then right and left
  quantum minors coincide, and we simply write $(i_1\ldots
  i_k|j_1\ldots j_k)$. This notation thus indicates
  that the sequences of numbers
  are increasing. In general, right and left quantum minors differ by
  a power of $-q$.
\item If two $i_l$'s or $j_l$'s coincide, then
  the quantum minors vanish.
\item The quantum determinant $\det_q$ is an
  element of the center of $A_q(n)$. 
\end{enumerate}
\end{rem}


\begin{defn}\label{defn:content}
  Let the \emph{content} of a monomial $x_{i_1j_1}\ldots x_{i_{m}j_{m}}$
  be defined as the tuple $(\alpha,\beta)=
  ((\alpha_1,\ldots,\alpha_n),(\beta_1,\ldots,\beta_n))$
  where $\alpha_i$
  is the number of indices $i_t$ such that $i_t=i$, and   $\beta_j$
  is the number of indices $j_t$ such that $j_t=j$. Note that
  $\sum\alpha_i=\sum\beta_j=m$ for each monomial of homogeneous
  degree $m$. For such a tuple $(\alpha,\beta)$,
  let $P(\alpha,\beta)$ be the subspace of $A_q(n,m)$ generated by the
  monomials of content $(\alpha,\beta)$. 
  Furthermore, let the \emph{content} of a bitableau
  $[\mathfrak{t},\mathfrak{t}']$
  be defined similarly as the
  tuple $(\alpha,\beta)$, such that $\alpha_i$ is the number of
  entries in $\mathfrak{t}$ equal to $i$ and  $\beta_j$ is the number of
  entries in $\mathfrak{t}'$ equal to $j$.
\end{defn}

\begin{thm}[\cite{huangzhang}]\label{thm:standardbasis}
  The bideterminants $(\mathfrak{t}|\mathfrak{t}')$ of the 
  standard $\lambda$-tableaux with  $\lambda$
  a partition of $m$ form a basis of $A_q(n,m)$, such that the
  bideterminants of standard $\lambda$-tableaux of content
  $(\alpha,\beta)$ form a basis of $P(\alpha,\beta)$.
\end{thm}
The proof  in \cite{huangzhang} works over a field,
but the arguments
are valid if the field is replaced by a commutative  ring with $1$.
The reversed order of the minors is due to the opposite algebra. Note
that for $i_1<i_2<\ldots<i_k$ and $j_1<j_2<\ldots<j_k$ we have 
\[ q^{\frac{k(k-1)}{2}}
(i_1i_2\ldots i_k|j_1j_2\ldots j_k)_r=
\sum_{w\in\mathfrak{S}_k}(-q)^{-l(w)}
   x_{i_{wk}j_{1}}x_{i_{w(k-1)}j_{2}}\ldots x_{i_{w1}j_{k}},
\]
which is a quantum minor of $A_{q^{-1}}(n)^{\mathrm{opp}}$. 

\begin{lem}[(Laplace's expansion \cite{huangzhang})]
  

  \begin{enumerate}
  \item  For $j_1<j_2<\ldots <j_l<j_{l+1}<\ldots <j_k$ we have
    \begin{align*}
      &(i_1i_2\ldots i_k|j_1j_2\ldots j_k)_l\\
      &=\sum_w (-q)^{l(w)}
      (i_1\ldots i_l|j_{w1}\ldots j_{wl})_l
      (i_{l+1}\ldots i_k|j_{w(l+1)}\ldots j_{wk})_l
    \end{align*} 
    where the summation is over all $w\in
    \mathfrak{S}_k $, such that $w1<w2<\ldots
    <wl$ and $w(l+1)<w(l+2)<\ldots <wk$.
\item
  For 
  $i_1<i_2<\ldots  <i_k$ we have
  \begin{align*}
    &(i_1i_2\ldots i_k|j_1j_2\ldots j_k)_r\\
    &=\sum_w (-q)^{l(w)}
    (i_{w1}\ldots i_{wl}|j_{1}\ldots j_{l})_r
    (i_{w(l+1)}\ldots i_{wk}|j_{l+1}\ldots j_{k})_r
  \end{align*} 
  the summation again over all $w\in
  \mathfrak{S}_k $, such that $w1<w2<\ldots
  <wl$ and $w(l+1)<w(l+2)<\ldots <wk$.
\end{enumerate}
\end{lem}


\section{$A_q(n;r,s)$} \label{sec:Aqnrs}
A basis of $\mathrm{End}_R(V^{\otimes r}\otimes {V^*}^{\otimes s})$ is
given by matrix units $E_{\mathbf i|\mathbf j\;\mathbf k|\mathbf l}$
such that $E_{\mathbf i|\mathbf j\;\mathbf k|\mathbf l}v_{\mathbf
  s|\mathbf t} = \delta_{\mathbf k|\mathbf l,\mathbf s|\mathbf
  t}v_{\mathbf i|\mathbf j}$.  Suppose $\varphi=\sum\limits_{\mathbf
  i,\mathbf j, \mathbf k, \mathbf l} c_{\mathbf i|\mathbf j\;\mathbf
  k|\mathbf l} E_{\mathbf i|\mathbf j\;\mathbf k|\mathbf l} \in
\mathrm{End}_R(V^{\otimes r}\otimes {V^*}^{\otimes s})$ commutes with
the action of $\mathfrak{B}_{r,s}^n(q)$ or equivalently with a set of
generators of $\mathfrak{B}_{r,s}^n(q)$.  Since coefficient spaces are
multiplicative, we can write
\[
c_{i_1k_1}c_{i_2k_2}\ldots c_{i_rk_r}
c_{j_1l_1}^*c_{j_2l_2}^*\ldots c_{j_sl_s}^*
\]
for the coefficient $c_{\mathbf i|\mathbf j\;\mathbf k|\mathbf l}$.
It is easy to see from the description of $A_q(n,m)$ that $\varphi$
commutes with the generators without non-propagating edges if and only
if the $c_{ij}$ satisfy the relations of $A_q(n)$ and the $c_{ij}^*$
satisfy the relations of $A_{q^{-1}}(n)$.

Now suppose that $\varphi$ in addition commutes with the action of the
generator 
\[e=\raisebox{-.1cm}{\epsfbox{si.20}}.\] 
We assume that $r=s=1$ (the general case being similar) and 
$\varphi=\sum\limits_{i,j,k,l=1}^n
c_{ik}c_{jl}^*E_{i|j\;k|l}$. 
 Let $v=v_i\otimes v_j^*$ be a basis element of
 $V\otimes V^*$.  We have (the indices in the sums always run 
 from $1$ to $n$)
\begin{eqnarray*}
  \varphi(v)e&=& \sum_{s, t} c_{si}c_{tj}^*(v_s\otimes v_t^*)e
  =  \sum_{s,k}q^{2s-n-1} c_{si}c_{sj}^*(v_k\otimes v_k^*)\\
   \varphi(ve)&=& \delta_{i j}q^{2i-n-1}\sum_{k}\varphi(v_k\otimes v_k^*)
  =\delta_{i j}q^{2i-n-1}\sum_{k,s,t}
  c_{sk}c_{tk}^*v_s\otimes v_t^*
\end{eqnarray*}

Comparing coefficients, we get the following conditions: 
\begin{gather*}
  \sum_{k=1}^n c_{ik}c_{jk}^*=0 \text{ for }i\neq j\\
  \sum_{k=1}^n q^{2k}c_{ki}c_{kj}^*=0 \text{ for }i\neq j\\
  \sum_{k=1}^n q^{2k-2i}c_{ki}c_{ki}^*=\sum_{k=1}^n c_{jk}c_{jk}^*.
\end{gather*}
This, combined with Lemma~\ref{lem:construction} shows that

\begin{lem}
  \[  A_q(n;r,s)\cong (F(n,r)\otimes_R F_*(n,s))/Y\]
  where $F(n,r)$ resp.~$F_*(n,s)$  is the $R$-submodule
   of the free algebra on generators $x_{ij}$ resp.~$x_{ij}^*$
   generated by monomials of degree
   $r$ resp.~$s$ and
   $Y$ is the $R$-submodule of 
   $F(n,r)\otimes_R F_*(n,s)$ generated by elements of the form
   $h_1h_2h_3$ where $h_2$ is one of the elements
  \begin{gather} 
    x_{ik}x_{jk}-qx_{jk} x_{ik}\text{ for }i<j
    \label{equ:A(nrs):1}\\
    x_{ki}x_{kj}-qx_{kj} x_{ki}\text{ for }i<j
    \label{equ:A(nrs):2}\\
    x_{ij}x_{kl}-x_{kl}x_{ij}\text{ for }i<k,j>l
    \label{equ:A(nrs):3}\\
    x_{ij}x_{kl}-x_{kl}x_{ij}-(q-q^{-1})x_{il}x_{kj}\text{ for
    }i<k,j<l
    \label{equ:A(nrs):4}\\
    x_{ik}^*x_{jk}^*-q^{-1}x_{jk}^* x_{ik}^*\text{ for }i<j
    \label{equ:A(nrs):5}\\
    x_{ki}^*x_{kj}^*-q^{-1}x_{kj}^* x_{ki}^*\text{ for }i<j
    \label{equ:A(nrs):6}\\
    x_{ij}^*x_{kl}^*-x_{kl}^*x_{ij}^*\text{ for }i<k,j>l
    \label{equ:A(nrs):7}\\
    x_{ij}^*x_{kl}^*-x_{kl}^*x_{ij}^*
    +(q-q^{-1})x_{il}^*x_{kj}^*\text{ for }i<k,j<l
    \label{equ:A(nrs):8}\\
    \sum_{k=1}^n x_{ik}x_{jk}^* \text{ for }i\neq j
    \label{equ:A(nrs):9}\\
    \sum_{k=1}^n q^{2k}x_{ki}x_{kj}^* \text{ for }i\neq j
    \label{equ:A(nrs):10}\\
    \sum_{k=1}^n q^{2k-2i}x_{ki}x_{ki}^*-\sum_{k=1}^n x_{jk}x_{jk}^* 
    \label{equ:A(nrs):11}
  \end{gather}
  and $h_1,h_3$ are monomials of appropriate degree.
\end{lem}

\begin{rem}\label{rem:automorphism}
  The map given by
  $x_{ik}\mapsto q^{2k-2i}x_{ki}$ and $x_{ik}^*\mapsto x_{ki}^*$
  induces an $R$-linear automorphism of $A_q(n;r,s)$.
\end{rem}


Bideterminants can also be formed using the variables $x_{ij}^*$. In
this case let
$(\mathfrak{t}|\mathfrak{t}')^*:=(\mathfrak{t}_1|\mathfrak{t}_1')_r^*
(\mathfrak{t}_2|\mathfrak{t}_2')_r^*\ldots
(\mathfrak{t}_k|\mathfrak{t}_k')_r^*$ where the quantum minors
$(i_1\ldots i_k|j_1\ldots j_k)_{r/l}^*$ are defined as above with $q$
replaced by $q^{-1}$.
   


\section{The map $\iota:A_q(n;r,s)\to A_q(n,r+(n-1)s)$}\label{sec:iota}
For any $1 \le i,j \le n$ let $\iota(x_{ij})=x_{ij}$ and 
\[\iota(x_{ij}^*)=
(-q)^{j-i}(12\ldots\hat{i}\ldots n|
12\ldots\hat{j}\ldots n)
\in A_q(n,n-1),\]
then there is a unique $R$-linear map
$\iota:F(n,r)\otimes_R F_*(n,s)\to
A_q(n,r+(n-1)s)$ such that $\iota(x_{i_1j_1}\ldots x_{i_rj_r}
x_{k_1l_1}^*\ldots x_{k_sl_s}^* )=\iota(x_{i_1j_1})\ldots \iota(x_{i_rj_r})
\iota(x_{k_1l_1}^*)\ldots \iota(x_{k_sl_s}^*)$. 
\begin{lem}\label{lem:factor}
  $\iota$ factors through $Y$ and thus induces an $R$-linear map 
  \[A_q(n;r,s)\to A_q(n,r+(n-1)s)\]
which we will then also denote by $\iota$. 
\end{lem}

\begin{proof}
  We have to show that the generators of $Y$ lie in the kernel of
  $\iota$.  Generators of $Y$ involving the elements
  \eqref{equ:A(nrs):1} up to \eqref{equ:A(nrs):4} are obviously in the
  kernel of $\iota$.  {\cite[Theorem~7.3]{goodearl}} shows that
  generators involving elements \eqref{equ:A(nrs):5} up to
  \eqref{equ:A(nrs):8} are also in the kernel.  Laplace's Expansion
  shows that
  \begin{eqnarray*}
    \iota\left(\sum_{k=1}^n x_{ik} x_{jk}^*\right)&=&
    \sum_{k=1}^n(-q)^{(k-1)-(j-1)}x_{ik}\cdot
    (1\ldots\hat{j}\ldots n|1\ldots\hat{k}\ldots n)_l\\
    &=&(-q)^{1-j}  (i1\ldots\hat{j}\ldots n|1\ldots n)_l
    = \delta_{i,j}\cdot{\det}_q \text{ and }\\ 
    \iota\left(\sum_{k=1}^n q^{2k-2i}x_{ki} x_{kj}^*\right)&=&
    q^{-2i+j+1}\sum_{k=1}^n(-q)^{k-1}x_{ki}\cdot
    (1\ldots\hat{k}\ldots n|1\ldots\hat{j}\ldots n)_r\\
    &=&(-q)^{j-2i+1}  (1\ldots n|i1\ldots\hat{j}\ldots n)_r
    = \delta_{i,j}\cdot{\det}_q,
\end{eqnarray*}
thus the generators involving the elements \eqref{equ:A(nrs):9} 
  up to \eqref{equ:A(nrs):11} are  in the kernel of $\iota$. 
\end{proof}


Now, we have maps 
\[
\iota^*: A_q(n,r+(n-1)s)^*\to A_q(n;r,s)^*\mbox{ and }
\pi:S_q(n,r+(n-1)s)\to S_q(n;r,s).\] By definition
$A_q(n,r+(n-1)s)^*\cong S_q(n,r+(n-1)s)$ and $A_q(n;r,s)^*\cong
S_q(n;r,s)$. Under these identifications we have

\begin{lem}
  $\iota^*=\pi.$
\end{lem}

\begin{proof}
  We will write $x_{i_1\ldots i_l\;j_1\ldots j_l}$
  instead of $x_{i_1,j_1}\ldots x_{i_l,j_l}$, 
   and  $x_{i_l\ldots i_1|l_1\ldots l_m\;j_l\ldots j_1|k_1\ldots
    k_m}$
  instead of 
  $x_{i_l,j_l}\ldots x_{i_1,j_1} x_{l_1,k_1}^*\ldots x_{l_m,k_m}^*$.
  Suppose that $\tilde\varphi\in A_q(n,r+(n-1)s)^*$. The
  corresponding element of $S_q(n,r+(n-1)s)$ is $\varphi=\sum\limits_{\mathbf
    i,\mathbf j\in \mathrm{I}(n,r+(n-1)s)} \tilde\varphi(x_{\mathbf
    i\mathbf j})E_{\mathbf i\mathbf j}$. Since
  $\iota^*(\tilde\varphi)=\tilde\varphi\circ\iota$, we have 
  \[\iota^*(\varphi)=
  \sum_{\mathbf i,\mathbf j,\mathbf k,\mathbf l}
  \tilde \varphi\circ\iota(x_{\mathbf i|\mathbf j\,\mathbf k|\mathbf l})
  E_{\mathbf i|\mathbf j\,\mathbf k|\mathbf l}\] 
  In other words: The coefficient of  
  $E_{\mathbf i|\mathbf j\,\mathbf k|\mathbf l} $ in
  $\iota^*(\varphi)$ can be computed by substituting each $x_{\mathbf
    s\mathbf t}$ in
  $\iota(x_{\mathbf i|\mathbf j\,\mathbf k|\mathbf l})$ by $\tilde\varphi(x_{\mathbf
    s\mathbf t})$.
  On the other hand, to compute the coefficient of 
  $E_{\mathbf i|\mathbf j\,\mathbf k|\mathbf l} $ in
  $\pi(\varphi)$, one has to
  consider the action of $\varphi$ on
  a basis element $v=\kappa(v_{\mathbf k|\mathbf l})$ of $T^{r,s}$. 
  For a multi index $\mathbf l\in\mathrm{I}(n,s)$ let $\mathbf
  l^*\in\mathrm{I}(n,(n-1)s)$ be defined by 
  \[\mathbf  l^*=(1\ldots\hat{l_1}\ldots n1\ldots\hat{l_2}\ldots
  n\ldots 1\ldots\hat{l_s}\ldots n ).\] 
  Then \[v=\kappa(v_{\mathbf k|\mathbf l})
  =(-q)^{l_1+l_2+\ldots +l_s}\sum_{w\in\mathfrak{S}_{n-1}^{\times
      s}}(-q)^{l(w)}
  v_{\mathbf k}\otimes(v_{\mathbf l^*}
  T_w)\]
  and thus we have
  \begin{eqnarray*}
    \varphi(v)&=&(-q)^{\sum l_k}\sum_{\mathbf s,\mathbf t,w}
    (-q)^{l(w)}\tilde\varphi(x_{\mathbf s\mathbf t})
    E_{\mathbf s\mathbf t}\left(v_{\mathbf k}\otimes (v_{\mathbf l^*}T_w)\right)\\
    &=&\sum_{\mathbf s,w}
    (-q)^{l(w)+\sum l_k}\tilde\varphi(x_{\mathbf s\;\mathbf k \mathbf l^*\!\!.w})
    v_{\mathbf s}.
  \end{eqnarray*}

  Since $\varphi$ leaves $T^{r,s}$ invariant, $\varphi(v)$ is a
  linear combination of the basis elements $\kappa(v_{\mathbf
    i|\mathbf j})$ of $T^{r,s}$. Distinct 
  $\kappa(v_{\mathbf i|\mathbf j})$ involve distinct basis vectors of
  $V^{\otimes r+(n-1)s}$. Thus if $\varphi(v)=
  \sum_{\mathbf i|\mathbf j} 
  \lambda_{\mathbf i|\mathbf j}\kappa(v_{\mathbf i|\mathbf j})=
  \sum_{\mathbf i|\mathbf j,w} 
  \lambda_{\mathbf i|\mathbf j}(-q)^{l(w)+j_1+\ldots+j_s}
  v_{\mathbf i\mathbf j^*.w}$  then
  $(-q)^{\sum j_k}\lambda_{\mathbf i|\mathbf j}$
  is equal to the coefficient of
  $v_{\mathbf i \mathbf j^*}$
  when $\varphi(v)$ is written as a linear
  combination of basis vectors of $V^{\otimes r+(n-1)s}$.
  The coefficient of 
  $v_{\mathbf i \mathbf j^*}$ in $\varphi(v)$ is, by the formula above, 
  \[(-q)^{\sum l_k}
  \sum_w(-q)^{l(w)}\tilde
  \varphi(x_{\mathbf i \mathbf j^*\;\mathbf k \mathbf l^*\!\!.w}).\]
  Thus 
  \[
  \lambda_{\mathbf i|\mathbf j}=
  (-q)^{\sum l_k-j_k}
  \sum_w(-q)^{l(w)}\tilde
  \varphi(x_{\mathbf i \mathbf j^*\;\mathbf k \mathbf l^*\!\!.w}) 
  =\tilde\varphi\circ\iota 
  (x_{\mathbf i|\mathbf j\;\mathbf k|\mathbf l}).
  \]
  But
  $\lambda_{\mathbf i|\mathbf j}$ is also the coefficient of
  $E_{\mathbf i|\mathbf j\;\mathbf k|\mathbf l }$ in $\pi(\varphi)$
  which shows the result.
\end{proof}


\begin{thm}[(Jacobi's Ratio Theorem)]\label{thm:jacobi}
  Suppose $n\geq l\geq 0$, 
  and $i_1<i_2<\ldots <i_l$ and $j_1<j_2<\ldots
  <j_l$. 
  Let $i_1'<i_2'<\ldots <i_{n-l}'$ and $j_1'<j_2'<\ldots <j_{n-l}'$
  be the unique numbers such that $\{1,\ldots,n\}=
  \{i_1,\ldots,i_l,i_1',\ldots,i_{n-l}'\}=
  \{j_1,\ldots,j_l,j_1',\ldots,j_{n-l}'\}$. Then 
  \[
  \iota\left((i_1\ldots i_l|j_1\ldots j_l)^*\right)
  =(-q)^{\sum_{t=1}^l (j_t-i_t)}\mathrm{det}_q^{l-1}
  (i_1' \ldots i_{n-l}'|j_1'\ldots j_{n-l}').
  \]
\end{thm}
\begin{proof}
We argue by induction on $l$. For $l=0$ we have
\[\iota(1)=1=\mathrm{det}_q^{-1}(1\ldots n|1\ldots n).\] 
For $l=1$ the theorem is true by the definition of
$\iota(x_{ij}^*)$. Now assume
the theorem is true for $l-1$. Apply Laplace's expansion and use
induction to get 
\begin{align*}
  \iota&\left((i_1\ldots i_l|j_1\ldots j_l)^*\right)
  =\iota\left(\sum_{k=1}^l(-q)^{-(k-1)}x_{i_kj_1}^* 
    (i_1\ldots\hat{i_k}\ldots i_l|j_2\ldots\ldots j_l)^*
  \right)\\
  &= \sum_{k=1}^l(-q)^{1-k}(-q)^{j_1-i_k}
  (1\ldots\hat{i_k}\ldots n|1\ldots\hat{j_1}\ldots n)\cdot
  (-q)^{\sum\limits_{t\neq1}j_t-\sum\limits_{t\neq k}i_t} 
    \mathrm{det}_q^{l-2}\\
    &\cdot(1\ldots\hat{i_1}\ldots\hat{i_2}\ldots\ldots\hat{i_{k-1}}
    \ldots\hat{i_{k+1}}\ldots\ldots\hat{i_l}\ldots n|
    1\ldots\hat{j_2}\ldots\hat{j_3}\ldots\ldots\hat{j_l}\ldots n)
\end{align*}
We claim that this is equal to 
\begin{align}
 (-q)^{\sum_{t=1}^l (j_t-i_t)}& \mathrm{det}_q^{l-2}
 \sum_w(-q)^{l(w)+1-n}
 (w1w2\ldots w(n-1)|1\ldots\hat{j_1}\ldots n)\notag\\
 & \cdot(wn\,1\ldots\hat{i_1}\ldots\ldots\hat{i_l}\ldots n|
 1\ldots\hat{j_2}\ldots\ldots\hat{j_l}\ldots n)_l\label{term:expansion}
\end{align}
where the summation is over all $w\in \mathfrak{S}_n$ such that
$w1<w2<\ldots <w(n-1)$. If $wn$ is not one of the $i_k$'s, then the
summand in (\ref{term:expansion}) vanishes, since $wn$ appears 
twice in the row on the left
side of the second minor. Thus the summation is over all $w$
as above with $wn=i_k$ for some $k$. Note that $l(w)=n-i_k$ and 
\[(i_k1\ldots\hat{i_1}\ldots\ldots\hat{i_l}\ldots n|\mathfrak{t})_l
=(-q)^{i_k-k}(1\ldots\hat{i_1}\ldots\hat{i_{k-1}}
\ldots\hat{i_{k+1}}\ldots\hat{i_l}\ldots n|
\mathfrak{t}),
\]
the claim follows. 
Again apply Laplace's expansion to the second minor in
(\ref{term:expansion}) to get
\begin{gather*}
  (wn\,1\ldots\hat{i_1}\ldots\ldots\hat{i_l}\ldots n|
  1\ldots\hat{j_2}\ldots\ldots\hat{j_l}\ldots n)_l\\
  =\sum_v(-q)^{l(v)}x_{wn\;v1} 
  (1\ldots\hat{i_1}\ldots\ldots\hat{i_l}\ldots n|
  v2v3\ldots\hat{vj_2}\ldots\ldots\hat{vj_l}\ldots vn),
\end{gather*}
the summation being over all $v\in
\mathfrak{S}_{\{1,\ldots,\hat{j_2},\ldots,\hat{j_l},\ldots,n\}}$ with
$v2<v3<\ldots <vn$. 
After substituting this term in (\ref{term:expansion}), one can again
apply Laplace's expansion, to get that
(\ref{term:expansion}) is equal to 
\begin{align}
  (-q)^{\sum(j_t-i_t)}& \mathrm{det}_q^{l-2}
  \sum_v(-q)^{l(v)+1-n} 
  (12\ldots n|1\ldots\hat{j_1}\ldots n\,v1)_r\notag\\
  & \cdot 
  (1\ldots\hat{i_1}\ldots\ldots\hat{i_l}\ldots n|
  v2v3\ldots\hat{vj_2}\ldots\ldots\hat{vj_l}\ldots vn)
  \label{term:expansion2}
\end{align}
The only summand in (\ref{term:expansion2}) that does not vanish, is
the term for $v1=j_1$ with $l(v)=j_1-1$.
Thus (\ref{term:expansion2}) is equal to 
\begin{align*}
  (-q&)^{\sum(j_t-i_t)}  \mathrm{det}_q^{l-2}
  (-q)^{j_1-n} 
  (12\ldots n|1\ldots\hat{j_1}\ldots nj_1)_r
  \cdot (i_1'\ldots i_{n-l}'|j_1'\ldots j_{n-l}')\\
  &=(-q)^{\sum_{t=1}^l (j_t-i_t)}\mathrm{det}_q^{l-1}
  (i_1'\ldots i_{n-l}'|j_1'\ldots j_{n-l}').
\end{align*}
\end{proof}




\section{A basis for $A_q(n;r,s)$}
Theorem~\ref{thm:jacobi} enables us to construct elements of
$A_q(n;r,s)$ that are mapped to standard bideterminants under $\iota$.
First, we will introduce the notion of rational tableaux, although we
will slightly differ from the definition of rational tableaux in
\cite{stembridge}. Recall that $\Lambda^+(k)$ is the set of partitions
of $k$. 
\begin{defn}\label{defn:rationaltableaux}
  A \emph{rational $(\rho,\sigma)$-tableau} is a pair
  $(\mathfrak{r},\mathfrak{s})$ such that $\mathfrak{r}$
  is a  $\rho$-tableau  and $\mathfrak{s}$ is a
  $\sigma$-tableau for some  $k\geq 0$,
  $\rho\in \Lambda^+(r-k)$ and $\sigma\in
  \Lambda^+(s-k)$ with $\rho_1+\sigma_1\leq n$.
  
  Let $\mathrm{first}_i(\mathfrak{r},\mathfrak{s})$ be the number 
  of entries of the first row of $\mathfrak{r}$ which are $\leq i$
  plus the number 
  of entries of the first row of $\mathfrak{s}$ which are $\leq i$. 
  A rational tableau is called \emph{standard} if 
  $\mathfrak{r}$ and $\mathfrak{s}$ are standard tableaux
  and the following condition  holds:
  \begin{equation}
    \mathrm{first}_i(\mathfrak{r},\mathfrak{s})\leq i 
    \text{ for all }i=1,\ldots,n
    \label{equ:condition}
  \end{equation}

  A pair $[(\mathfrak{r},\mathfrak{s}),
  (\mathfrak{r}',\mathfrak{s}')]$ of rational
  $(\rho,\sigma)$-tableaux is
  called a \emph{rational  bitableau},
  and it is called a
  standard rational bitableau if both 
  $(\mathfrak{r},\mathfrak{s})$ and 
  $(\mathfrak{r}',\mathfrak{s}')$ are
  standard rational tableaux. 
\end{defn}

\begin{rem}
  In \cite{stembridge}, condition~\eqref{equ:condition} is already
  part of the definition of rational tableaux.  The condition
  $\rho_1+\sigma_1\leq n$ is equivalent to
  condition~\eqref{equ:condition} for $i=n$. The reason for the
  difference will be apparent in the proof of the next lemma. 
\end{rem}


\begin{lem}\label{lem:bijection}
  There is a bijection between the set consisting of all standard
  rational $(\rho,\sigma)$-tableaux for $\rho\in \Lambda^+(r-k)$,
  $\sigma\in \Lambda^+(s-k)$, as $k$ runs from 0 to $\min(r,s)$ and
  the set of all standard $\lambda$-tableaux for
  $\lambda\in\Lambda^+(r+(n-1)s)$ satisfying $\sum_{i=1}^s\lambda_i
  \geq (n-1)s$.
\end{lem}

\begin{proof}
  Given a rational $(\rho,\sigma)$-tableau 
  $(\mathfrak{r},\mathfrak{s})$ we construct a
  $\lambda$-tableau $\mathfrak{t}$ as follows: 
  Draw a rectangular diagram with $s$ rows and $n$ columns. Rotate the
  tableau $\mathfrak{s}$ by 180 degrees and place 
  it in the bottom right corner
  of the  rectangle. Place the tableau $\mathfrak{r}$
  on the left side
  below the
  rectangle. Fill the empty boxes of the rectangle with numbers, such
  that in each row, the entries that do not appear in 
  $\mathfrak{t}$ appear in
  the empty boxes in increasing order. Let $\mathfrak{t}$ be the tableau
  consisting of the formerly empty boxes
  and the boxes of $\mathfrak{r}$.  We
  illustrate this procedure with an example. Let
  $n=5,r=4,s=5,k=1$. Then \Yvcentermath1
  \[ 
  (\mathfrak{r},\mathfrak{s})=
  \left(\young(13,2),\young(34,35)
  \right)
  \leadsto\young(\hfill\hfill\hfill\hfill\hfill 
  ,\hfill\hfill\hfill\hfill\hfill 
  ,\hfill\hfill\hfill\hfill\hfill
  ,\hfill\hfill\hfill 53,\hfill\hfill\hfill 43,13,2)
  \leadsto
  \young(12345,12345,12345,12453,12543,13,2)
  \leadsto \mathfrak{t}= 
  \young(12345,12345,12345,124,125,13,2)
  \]
  It is now easy to give an inverse: Just draw the rectangle into the
  tableau $\mathfrak{t}$, fill the empty boxes of the rectangle in a
  similar way as before, rotate these back to obtain
  $\mathfrak{s}$. $\mathfrak{r}$ is the part of the tableau
  $\mathfrak{t}$, that lies outside the rectangle.  We have to show,
  that these bijections provide standard tableaux of the right shape.

  Suppose $(\mathfrak{r},\mathfrak{s})$ 
  is a rational $(\rho,\sigma)$-tableau,
  then $\mathfrak{t}$ is a $\lambda$-tableau,
  with $\lambda_i=n-\sigma_{s+1-i}$
  for $i\leq s$ and $\lambda_i=\rho_{i-s}$ for $i>s$. Thus
  $\lambda_i\geq \lambda_{i+1}$ for $i<s$ is equivalent to 
  $\sigma_{s+1-i}\leq \sigma_{s-i}$, and for $i>s$ it is equivalent to
  $\rho_{i-s}\geq \rho_{i+1-s}$. Now  $\rho_1+\sigma_1=
  \lambda_{s+1}-(\lambda_{s}-n)$. This shows that $\lambda$ is a
  partition if and only if $\rho$ and $\sigma$ are partitions with
  $\rho_1+\sigma_1\leq n$.
  We still have to show that 
  $(\mathfrak{r},\mathfrak{s})$ is standard if and only
  if $\mathfrak{t}$ is standard. 

  By definition, all standard tableaux have increasing
  rows. A tableau has nondecreasing columns if and only if for all
  $i=1,\ldots, n$ and all rows (except for the last row)
  the number of  entries $\leq i$ in this row is greater or equal than 
  the number of  entries $\leq i$ in the next row. Now, it follows
  from the construction that $\mathfrak{t}$ 
  has nondecreasing columns inside the
  rectangle if and only if $\mathfrak{s}$ has  nondecreasing columns,
  $\mathfrak{t}$ has nondecreasing columns outside the
  rectangle if and only if $\mathfrak{r}$
  has  nondecreasing columns, and the
  columns in $\mathfrak{t}$ do not decrease
  from row $s$ to row $s+1$ if and only
  if condition~\eqref{equ:condition} holds. 
\end{proof}


\begin{defn}
  For $ k\geq 1$ let $\mathfrak{det}_q^{(k)}
  \in A_q(n;k,k)$ be recursively defined by
  $\mathfrak{det}_q^{(1)}:=\sum_{l=1}^n x_{1l}x_{1l}^*$ and
  $\mathfrak{det}_q^{(k)}:=
  \sum_{l=1}^n x_{1l}\mathfrak{det}_q^{(k-1)}x_{1l}^* $ for $k>1$.

  
  Let a (rational) bideterminant 
  $\left((\mathfrak{r},\mathfrak{s})|
    (\mathfrak{r}',\mathfrak{s}')\right)\in
  A_q(n;r,s)$ be defined by 
  \[\left((\mathfrak{r},\mathfrak{s})|
    (\mathfrak{r}',\mathfrak{s}')\right):=
  (\mathfrak{r}|\mathfrak{r}')\;
  \mathfrak{det}_q^{(k)}\;(\mathfrak{s}|\mathfrak{s}')^*\]
  whenever $[(\mathfrak{r},\mathfrak{s}),
  (\mathfrak{r}',\mathfrak{s}')]$ is a 
  rational  $(\rho,\sigma)$-bitableau
  such that $\rho\in \Lambda^+(r-k)$, $\sigma\in
  \Lambda^+(s-k)$, for some $k = 0, 1, \dots, \min(r,s)$.
\end{defn}

Note that the proof of Lemma~\ref{lem:factor} shows that
$\iota(\mathfrak{det}_q^{(k)})=\mathrm{det}_q^k$. 
Furthermore, if $\rho_1$ or $\sigma_1>n$, then the bideterminant of a
$(\rho,\sigma)$-bitableau vanishes. 
As a direct  consequence of Theorem~\ref{thm:jacobi} we get
\begin{lem}
  Let $(\mathfrak{r},\mathfrak{s})$ and 
  $(\mathfrak{r}',\mathfrak{s}')$ be 
  two standard rational tableaux, and let $\mathfrak{t}$
  and $\mathfrak{t}'$ be the (standard) tableaux obtained 
  from the correspondence of
  Lemma~\ref{lem:bijection}. Then we have
  \[
  \iota((\mathfrak{r},\mathfrak{s})|(\mathfrak{r}',\mathfrak{s}'))
  =(-q)^{c(\mathfrak{t},\mathfrak{t}')}
  (\mathfrak{t}|\mathfrak{t}')
  \]
  for some integer ${c(\mathfrak{t},\mathfrak{t}')}$.
  In particular, the bideterminants of standard rational bitableaux
  are linearly independent.  
\end{lem}
\begin{proof}
This follows directly from Theorem~\ref{thm:jacobi}, the construction
of the bijection and
$\iota(\mathfrak{det}_q^{(k)})=\mathrm{det}_q^k$. The second
statement follows from the fact that the 
$(\mathfrak{t}|\mathfrak{t}')$'s are linearly
independent. 
\end{proof}

\begin{lem}\label{lem:detk}
We have 
\begin{gather}
  \sum_{l=1}^n x_{il}\mathfrak{det}_q^{(k)}x_{jl}^*
  =0\text{ for }i\neq j\label{equ:det1}\\
  \sum_{l=1}^n q^{2l}x_{li}\mathfrak{det}_q^{(k)}x_{lj}^*
    =0\text{ for }i\neq j
  \label{equ:det2}\\
  \sum_{l=1}^n q^{2l-2i}x_{li}\mathfrak{det}_q^{(k)}x_{li}^*=
  \sum_{l=1}^n x_{jl}\mathfrak{det}_q^{(k)}x_{jl}^*\label{equ:det3}
\end{gather}
\end{lem}
\begin{proof}Without loss of generality, we may assume that $k=1$. 
  Suppose  that $i,j\neq 1$. Then
  \begin{align*}
    \sum_{l=1}^n& x_{il}\mathfrak{det}_q^{(1)}x_{jl}^*=
    \sum_{k,l=1}^n x_{ik}x_{1l}x_{1l}^*x_{jk}^*
    =\sum_{k<l} x_{1l}x_{ik}x_{jk}^*x_{1l}^*
    +q^{-2}\sum_{k} x_{1k}x_{ik}x_{jk}^*x_{1k}^*\\
    &+\sum_{k>l} \left(x_{1l}x_{ik}x_{jk}^*x_{1l}^*
      +(q^{-1}-q)(x_{1k}x_{il}x_{1l}^*x_{jk}^*+
      x_{1l}x_{ik}x_{1k}^*x_{jl}^* ) \right)\\
    &=\sum_{k,l} x_{1l}x_{ik}x_{jk}^*x_{1l}^*
    +(q^{-2}-1)\sum_{k} q x_{1k}x_{ik}x_{1k}^*x_{jk}^*\\
    &+(q^{-1}-q)\sum_{k>l}(x_{1k}x_{il}x_{1l}^*x_{jk}^*+
    x_{1l}x_{ik}x_{1k}^*x_{jl}^* )\\
    &=\delta_{ij}\mathfrak{det}_q^{(2)}
    +(q^{-1}-q)\sum_{k,l}x_{1k}x_{il}x_{1l}^*x_{jk}^*
    =\delta_{ij}\mathfrak{det}_q^{(2)} .
  \end{align*}
For $j\neq 1$ we have 
\begin{align*}
    \sum_{l=1}^n& x_{1l}\mathfrak{det}_q^{(1)}x_{jl}^*=
    \sum_{k,l=1}^n x_{1k}x_{1l}x_{1l}^*x_{jk}^*
    =\sum_{k<l} qx_{1l}x_{1k}x_{jk}^*x_{1l}^*
    +q^{-1}\sum_{k} x_{1k}x_{1k}x_{jk}^*x_{1k}^*\\
    &+\sum_{k>l} \left(q^{-1}x_{1l}x_{1k}x_{jk}^*x_{1l}^*
      +(q^{-1}-q) x_{1k}x_{1l}x_{jl}^*x_{1k}^*\right)\\
    &=\sum_{k,l} q^{-1}x_{1l}x_{1k}x_{jk}^*x_{1l}^*=0.
  \end{align*}
Similarly, one can show that
\begin{eqnarray*}
   \sum_{l=1}^n x_{il}\mathfrak{det}_q^{(1)}x_{1l}^*
   &=&0\text{ for }i\neq 1\\
   \sum_{l=1}^n q^{2l-2i}x_{li}\mathfrak{det}_q^{(1)}x_{lj}^*
   &=&\delta_{ij}\sum_{l=1}^n q^{2l-2}x_{l1}
   \mathfrak{det}_q^{(1)}x_{l1}^*
   \text{ for }i,j\neq 1\\
   \sum_{l=1}^n q^{2l-2}x_{l1}\mathfrak{det}_q^{(1)}x_{lj}^*
   &=&0\text{ for }j\neq 1\\ 
   \sum_{l=1}^n q^{2l-2i}x_{li}\mathfrak{det}_q^{(1)}x_{l1}^*
   &=&0\text{ for }i\neq 1.\\
\end{eqnarray*}
Finally, 
\begin{align*}
  \sum_{l=1}^n &q^{2l-2}x_{l1}\mathfrak{det}_q^{(1)}x_{l1}^*
  =\sum_{l,k} q^{2l-2}x_{l1} x_{1k} x_{1k}^*x_{l1}^*
  =\sum_{l,k\neq 1} q^{2l-2} x_{1k}x_{l1}x_{l1}^* x_{1k}^*\\
  &+\sum_{l\neq 1} q^{2l-4} x_{11}x_{l1}x_{l1}^* x_{11}^*
  +\sum_{k\neq 1} q^{2} x_{1k}x_{11}x_{11}^* x_{1k}^*
  + x_{11}x_{11}x_{11}^* x_{11}^*\\
  &=\mathfrak{det}_q^{(2)}
  +\sum_{l\neq 1} q^{2l-4}(1-q^2) x_{11}x_{l1}x_{l1}^* x_{11}^*
  +\sum_{k\neq 1} (q^{2}-1) x_{1k}x_{11}x_{11}^* x_{1k}^*\\
  &=\mathfrak{det}_q^{(2)}+(1-q^2)\left(
    \sum_{l\neq 1} q^{2l-4} x_{11}x_{l1}x_{l1}^* x_{11}^*
    -q^{-2}\sum_{k\neq 1} x_{11}x_{1k}x_{1k}^* x_{11}^*\right)
  =\mathfrak{det}_q^{(2)}.
\end{align*}
The proof is complete.
\end{proof}

\begin{lem}\label{lem:straightening}
  Suppose $\mathbf r=(r_1,\ldots,r_k),\mathbf s=(s_1,\ldots,s_k)\in
  I(n,k)$ are fixed. 
%  For $j_1,\ldots,j_k\in\{1,\ldots,n\}$ let
%  \[
%  x(j_1,\ldots,j_k):=(\mathbf r|j_k\ldots j_2j_1)_r(\mathbf
%  s|j_1j_2\ldots j_k)_r^*. 
%  \]
  Let $j\in\{1,\ldots,n\}$ and $k\geq 1$. 
  Then we have, modulo $\mathfrak{det}_q^{(1)}$,
  \begin{eqnarray*}
  &\sum\limits_{j<j_1<j_2<\ldots <j_k}&(\mathbf r|j_k\ldots j_2j_1)_r(\mathbf
  s|j_1j_2\ldots j_k)_r^*\\%x(j_1j_2\ldots j_k)
  &&\equiv(-1)^kq^{2\sum_{i=0}^{k-1}i}\sum_{j_1<j_2<\ldots <j_k\leq j}
  (\mathbf r|j_k\ldots j_2j_1)_r(\mathbf
  s|j_1j_2\ldots j_k)_r^*%x(j_1j_2\ldots j_k) .
  \end{eqnarray*}
\end{lem}

\begin{proof}
$(\mathbf s|j_1j_2\ldots j_k)_r^*$ and
$(\mathbf s|j_1j_2\ldots j_k)_l^*$ differ only on a power of $-q$
not depending on $j_1,j_2,\ldots,j_k$. Thus we can show the lemma with 
$(\_,\_)_r^*$ replaced by
$(\_,\_)_l^*$. Similarly, we can assume that $r_1<r_2<\ldots <r_k$
and $s_1>s_2>\ldots >s_k$. 
Note that modulo $\mathfrak{det}_q^{(1)}$  we have the relations 
$\sum_{k=1}^n x_{ik}x_{jk}^* \equiv0$.
It follows that the lemma is
true for $k=1$.
Assume that the lemma holds for $k-1$. 
If $M$ is an ordered set, let $M^{k,<}$ be the set of 
$k$-tuples in $M$ with increasing entries. 
For a subset
$M\subset \{1,\ldots,n\}$ we have 
\begin{align*}
  \sum_{\mathbf j\in M^{k,<}}&(\mathbf r|j_k\ldots j_2j_1)_r(\mathbf
  s|j_1j_2\ldots j_k)_l^*\\
  &=
  \sum_{\mathbf j\in M^{k,<},w}(-q)^{-l(w)}
  (\mathbf r|j_k\ldots j_2j_1)_r
  x_{s_1j_{w1}}^*\ldots x_{s_kj_{wk}}^*\\
  &= \sum_{\mathbf j\in M^{k,<},w}
  (\mathbf r|j_{wk}\ldots j_{w1})_r
  x_{s_1j_{w1}}^*\ldots x_{s_kj_{wk}}^*\\
  &= \sum_{\mathbf j\in M^k}
  (\mathbf r|j_{k}\ldots j_{1})_r
  x_{s_1j_{1}}^*\ldots x_{s_kj_{k}}^*
\end{align*}
Applying Laplace's Expansion, we can write
a quantum minor $(\mathbf r|\mathbf j_1\mathbf j_2)_r$ as a linear
combination of products of quantum minors, say 
$(\mathbf r|\mathbf j_1\mathbf j_2)_r
=\sum_lc_l(\mathbf r'_l|\mathbf j_1)_r(\mathbf r''_l|\mathbf j_2)_r$.
Then with $\epsilon_k:=(-1)^kq^{2\sum_{i=0}^{k-1}i}$, 
$\mathbf j=(j_1,\ldots,j_k)$ and 
$\mathbf j'=(j_1,\ldots,j_{k-1})$, $D=\{j+1\ldots n\}$ and
$C=\{1\ldots  j\}$, we have
 
\begin{align*}
  \sum_{\mathbf j\in D^{k,<}}&(\mathbf r|j_k\ldots j_2j_1)_r(\mathbf
  s|j_1j_2\ldots j_k)_l^*
  =\sum_{\mathbf j\in D^{k}}
  (\mathbf r|j_{k}\ldots j_{1})_r
  x_{s_1j_{1}}^*\ldots x_{s_kj_{k}}^*\\
  &=\sum_{\mathbf j\in D^{k},l}
  c_l(\mathbf r'_l|j_{k})_r(\mathbf r''_l|j_{k-1}\ldots j_{1})_r
  x_{s_1j_{1}}^*\ldots x_{s_{k-1}j_{k-1}}^*x_{s_kj_{k}}^*\\
  &\equiv\epsilon_{k-1}
  \sum_{\genfrac{}{}{0pt}{}{\mathbf j'\in C^{k-1},l}{j_k>j}}
  c_l(\mathbf r'_l|j_{k})_r(\mathbf r''_l|j_{k-1}\ldots j_{1})_r
  x_{s_1j_{1}}^*\ldots x_{s_{k-1}j_{k-1}}^*x_{s_kj_{k}}^*\\
  &=\epsilon_{k-1}
  \sum_{\genfrac{}{}{0pt}{}{\mathbf j'\in C^{k-1}}{j_k>j}}
  (\mathbf r|j_{k}j_{k-1}\ldots j_{1})_r
  x_{s_1j_{1}}^*\ldots x_{s_{k-1}j_{k-1}}^*x_{s_kj_{k}}^*\\
  &=\epsilon_{k-1}
  \sum_{\genfrac{}{}{0pt}{}{\mathbf j'\in C^{k-1}}{j_k>j}}
  (-q)^{k-1}
  (\mathbf r|j_{k-1}\ldots j_{1}j_{k})_r
  x_{s_kj_{k}}^*x_{s_1j_{1}}^*\ldots x_{s_{k-1}j_{k-1}}^*\\
  &=\epsilon_{k-1}
  \sum_{\genfrac{}{}{0pt}{}{\mathbf j'\in C^{k-1},l}{j_k>j}}
  (-q)^{k-1}
  c_l(\mathbf r_l'|j_{k-1}\ldots j_{1})_rx_{\mathbf r_l''j_{k}}
  x_{s_kj_{k}}^*x_{s_1j_{1}}^*\ldots x_{s_{k-1}j_{k-1}}^*\\
  &\equiv-\epsilon_{k-1}
  \sum_{\mathbf j\in C^{k},l}
  (-q)^{k-1}
  c_l(\mathbf r_l'|j_{k-1}\ldots j_{1})_rx_{\mathbf r_l''j_{k}}
  x_{s_kj_{k}}^*x_{s_1j_{1}}^*\ldots x_{s_{k-1}j_{k-1}}^*\\
  &=-\epsilon_{k-1}
  \sum_{\mathbf j\in C^{k}}
  (-q)^{k-1}
  (\mathbf r|j_{k-1}\ldots j_{1}j_{k})_r
  x_{s_kj_{k}}^*x_{s_1j_{1}}^*\ldots x_{s_{k-1}j_{k-1}}^*\\
  &=-\epsilon_{k-1}
  \sum_{\mathbf j\in C^{k,<}}
  (-q)^{k-1}
  (\mathbf r|j_{k}\ldots j_{1})_r
  (s_ks_1\ldots s_{k-1}|j_1\ldots j_{k})_l^*
  \\
  &=-\epsilon_{k-1}
  \sum_{\mathbf j\in C^{k,<}}
  (-q)^{2(k-1)}
  (\mathbf r|j_{k}\ldots j_{1})_r
  (s_1\ldots s_k|j_1\ldots j_{k})_l^*\\
  &=\epsilon_k\sum_{\mathbf j\in C^{k,<}}
  (\mathbf r|j_k\ldots j_2j_1)_r(\mathbf
  s|j_1j_2\ldots j_k)_l^* 
\end{align*}
and the proof is complete.
\end{proof}

\begin{lem}\label{lem:straightening2}
Let $\mathbf r'$ and $\mathbf s'$ be strictly increasing 
multi indices, considered as
tableaux with one row. Let $i$ be the maximal entry appearing 
and suppose that  $i$ is minimal such
that $i$ violates condition~\eqref{equ:condition}.
Let $I$ be the set of entries appearing in both  $\mathbf r'$ and
$\mathbf s'$, then we have $i\in I$. Let $L_1=\{k_1,\ldots,k_{l_1}\}$ 
(resp.~$L_2=\{k_1',\ldots,k_{l_2}'\}$)
be the set of entries of $\mathbf r'$ (resp.~$\mathbf s'$) not
appearing in $\mathbf s'$(resp.~$\mathbf r'$), and let $i_1<i_2<\ldots
<i_k=i$ be the entries of $I$.
Let $D=\{i_1,\ldots,i_k,i_k+1,i_k+2,\ldots,n\}$ and
$C=\{1,\ldots,n\}\backslash (D\cup L_1\cup L_2)$. Furthermore,
for $j_1,\ldots,j_t\in \{1,\ldots,n\}$ let 
\[m(j_1,\ldots,j_t)=|\{(l,c)\in\{1,\ldots,t\}\times
C:j_l<c\}|.\]
Let $\mathbf
k=(k_1,\ldots,k_{l_1}), \mathbf k'=(k_1',\ldots,k_{l_2}')$
and let $\mathbf r$ and $\mathbf s$ be multi indices of the same
length as $\mathbf r'$ resp.~$\mathbf s'$, then
we have  
\[
\sum_{\mathbf j\in D^{k,<}}
q^{2m(\mathbf j)}
(\mathbf r|\mathbf k j_k\ldots j_1)_r
(\mathbf s|j_1\ldots j_k \mathbf k' )_r^*
\equiv0\text{ modulo }\mathfrak{det}_q^{(1)}.
\]
\end{lem}

\begin{proof}
  Note that $i\in I$ and $i=2k+l_1+l_2-1$, otherwise $i-1$ would violate 
  condition~\eqref{equ:condition}. Thus $|C|=k-1$.
  Let $c_{max}$ be the 
  maximal element of $C$, 
  $\tilde{D}=\{c_{max}+1,c_{max}+2,\ldots,n\}
  \subset D\cup L_1\cup L_2$, $\tilde{C}=\{1,\ldots,c_{max}\}$, 
  $D_-=\{d\in D:d<c_{max}\}$ and 
  $D_+=\{d\in D:d>c_{max}\}$. With 
  $\tilde{\mathbf j}=(j_1,\ldots, j_l)$ and 
  $\hat{\mathbf j}=(j_{l+1},\ldots, j_k)$ we have 
  \begin{align}
    \sum_{\mathbf j\in D^{k,<}}&
    q^{2m(\mathbf j)}
    (\mathbf r|\mathbf k j_k\ldots j_1)_r
    (\mathbf s|j_1\ldots j_k \mathbf k' )_r^*\notag\\
    &=\sum_{l=0}^k
    \sum_{\tilde{\mathbf j}\in D_-^{l,<}}
    q^{2m(\tilde{\mathbf j})}
    \sum_{\hat{\mathbf j}\in D_+^{k-l,<}}
    (\mathbf r|\mathbf k j_k\ldots j_1)_r
    (\mathbf s|j_1\ldots j_k \mathbf k' )_r^* .
    \label{equ:xj}
  \end{align}
  Without loss of generality we may assume that the entries in
  $\mathbf s$ are increasing. 
  We apply Laplace's Expansion and 
  Lemma~\ref{lem:straightening} to get 
  for fixed $l$ and $\tilde{\mathbf j}$
  \begin{align*}
    \sum_{\hat{\mathbf j}\in D_+^{k-l,<}}&
    (\mathbf r|\mathbf k j_k\ldots j_1)_r
    (\mathbf s|j_1\ldots j_k \mathbf k' )_r^*
    =\sum_{\hat{\mathbf j}\in \tilde{D}^{k-l,<}}
    (\mathbf r|\mathbf k j_k\ldots j_1)_r
    (\mathbf s|j_1\ldots j_k \mathbf k' )_r^*\\
    &=q^{2l(k-l)}
    \sum_{\hat{\mathbf j}\in \tilde{D}^{k-l,<}}
    (\mathbf r|\mathbf k j_l\ldots j_1j_k\ldots j_{l+1})_r
    (\mathbf s|j_{l+1}\ldots j_k j_1\ldots j_l\mathbf k')_r^*\\
    &\equiv\epsilon_{k-l}q^{2l(k-l)}
    \sum_{\hat{\mathbf j}\in \tilde{C}^{k-l,<}}
    (\mathbf r|\mathbf k j_l\ldots j_1j_k\ldots j_{l+1})_r
    (\mathbf s|j_{l+1}\ldots j_k j_1\ldots j_l\mathbf k')_r^*\\
    &=\epsilon_{k-l}q^{2l(k-l)}
    \sum_{\hat{\mathbf j}\in (C\cup D_-)^{k-l,<}}
    (\mathbf r|\mathbf k j_l\ldots j_1j_k\ldots j_{l+1})_r
    (\mathbf s|j_{l+1}\ldots j_k j_1\ldots j_l\mathbf k')_r^* .
  \end{align*}
  This expression can be substituted into \eqref{equ:xj}. 
  Each nonzero summand belongs to a disjoint union 
  $S_1\dot\cup S_2=S\subset C\cup D_-$ with $|S|=k$, 
  $S_1=\{j_1,\ldots,j_l\}$ and $S_2=\{j_{l+1},\ldots,j_k\}$. 
  We will show that the summands belonging to some fixed set $S$
  cancel out. 

  Therefore, we claim that for each subset $S\subset C\cup D_-$ 
  with $k$ elements
  there exists some $d\in D\cap S$ such that 
  $m(d)=|\{s\in S:s>d\}|$.  Suppose not.
  $S$ contains at least one element of $D$
  since $|C|=k-1$. 
  Let $s_1<s_2<\ldots <s_m$ be the elements 
  of $D\cap S$. We show by downward induction that 
  $m(s_l)>|\{s\in S:s>s_l\}|$ for  $1\leq l\leq m$:
  $m(s_m)$ is
  the cardinality of 
  $\{s_m+1,\ldots,c_{max}\}\cap C$.
  Since all $s\in S$ with $s>s_m$ are elements of $C$ we have 
  $\{s_m+1,\ldots,c_{max}\}\cap S\subset 
  \{s_m+1,\ldots,c_{max}\}\cap C$, and thus 
  $m(s_m)\geq|\{s\in S:s>s_m\}|$. By assumption we have
  $>$ instead of $\geq$. 
  Suppose now, that 
  $m(s_l)>|\{s\in S:s>s_l\}|$. 
  We have $\{s\in S:s_{l-1}<s\leq s_l\}=
  \{s\in S\cap C:s_{l-1}<s< s_l\}\cup\{s_l\}$, thus $S$
  contains at most $m(s_{l-1})-m(s_l)$
  elements between  $s_{l-1}$ and $s_l$, and thus at most 
  $m(s_{l-1})-m(s_l)+1+m(s_l)-1
  =m(s_{l-1})$ elements $>s_{l-1}$. By assumption we have 
  $m(s_{l-1})>|\{s\in S:s>s_{l-1}\}|$.
  We have shown that $S$ contains less than $m(s_1)$
  elements greater than $s_1$,
  thus $S$ contains less than  $ |C|+1=k$ elements
  which is a contradiction. This shows the claim. 

  Let $S\subset C\cup D_-$ be fixed subset of cardinality $k$. 
  By the previous consideration there is an element $d\in D\cap S$
  with $m(d)=|\{s\in S:s>d\}|$.
  We claim that the summand
  for $S_1,S_2$ with $d\in S_1$ cancels the summand for   
  $S_1\backslash\{d\},S_2\cup\{d\}$. 
  Note that
  \begin{align*}
    (\mathbf r|&\mathbf k j_l\ldots\hat{d}
    \ldots j_1j_k\ldots{d}\ldots j_{l+1})_r
    (\mathbf s|j_{l+1}\ldots{d}\ldots j_k
    j_1\ldots\hat{d}\ldots j_l\mathbf k')^*_r\\
    &= q^{2|\{s\in S:s>d\}|-2(l-1)}
    (\mathbf r|\mathbf k j_l\ldots j_1j_k\ldots j_{l+1})_r
    (\mathbf s|j_{l+1}\ldots j_kj_1\ldots j_l\mathbf k')^*_r .
  \end{align*}
  Comparing coefficients, we see that both summands cancel. 
\end{proof}





\begin{thm}[(Rational Straightening Algorithm)]
  The set of bideterminants of standard rational bitableaux forms an
  $R$-basis of $A_q(n;r,s)$.  
\end{thm}
\begin{proof}
  We have to show that the bideterminants of standard rational
  bitableaux generate $A_q(n;r,s)$.  Clearly, the bideterminants
  $((\mathfrak{r},\mathfrak{s})|(\mathfrak{r}',\mathfrak{s}'))$ with
  $\mathfrak{r},\mathfrak{r}',\mathfrak{s},\mathfrak{s}'$ standard
  tableaux generate $A_q(n;r,s)$.  Let $\mathrm{cont}(\mathfrak{r})$
  resp.~$\mathrm{cont}(\mathfrak{s})$ be the content of $\mathfrak{r}$
  resp.~$\mathfrak{s}$ defined in Definition~\ref{defn:content}.
  
  For standard tableaux
  $\mathfrak{r},\mathfrak{r}',\mathfrak{s},\mathfrak{s}'$ such that
  the rational bitableau
  $[(\mathfrak{r},\mathfrak{s}),(\mathfrak{r}',\mathfrak{s}')]$ is not
  standard, it suffices to show that the bideterminant
  $((\mathfrak{r},\mathfrak{s})|(\mathfrak{r}',\mathfrak{s}'))$ is a
  linear combination of bideterminants
  $((\hat{\mathfrak{r}},\hat{\mathfrak{s}})|
  (\hat{\mathfrak{r}}',\hat{\mathfrak{s}}'))$ such that
  $\hat{\mathfrak{r}}$ has fewer boxes than $\mathfrak{r}$ or
  $\mathrm{cont}(\mathfrak{r})>\mathrm{cont}(\hat{\mathfrak{r}})$ or
  $\mathrm{cont}(\mathfrak{s})>\mathrm{cont}(\hat{\mathfrak{s}})$ in
  the lexicographical order.  Without loss of generality we make the
  following assumptions:
  \begin{itemize}
  \item In the nonstandard rational bitableau
    $[(\mathfrak{r},\mathfrak{s}),(\mathfrak{r}',\mathfrak{s}')]$, the
    rational tableau $(\mathfrak{r}',\mathfrak{s}')$ is
    nonstandard. Note that the automorphism of
    Remark~\ref{rem:automorphism} maps a bideterminant
    $((\mathfrak{r},\mathfrak{s})|(\mathfrak{r}',\mathfrak{s}'))$ to
    the bideterminant
    $((\mathfrak{r}',\mathfrak{s}')|(\mathfrak{r},\mathfrak{s}))$.
  \item Suppose that $(\mathfrak{r},\mathfrak{s})$ 
    and $(\mathfrak{r}',\mathfrak{s}')$ are
    $(\rho,\sigma)$-tableaux. In view of Lemma~\ref{lem:detk} we can
    assume that  $\rho\in \Lambda^+(r)$ and
    $\sigma\in\Lambda^+(s)$. 
  \item $\mathfrak{r},\mathfrak{r}',\mathfrak{s},\mathfrak{s}'$
    are tableaux with only one row (each bideterminant 
    has a factor of this type, and we can use
    Theorem~\ref{thm:standardbasis} to write nonstandard
    bideterminants as a linear combination of standard ones of the
    same content. 
  \item Let $i$ be minimal such that condition~\eqref{equ:condition} of 
    Definition~\ref{defn:rationaltableaux}   is violated for $i$. 
    Applying Laplace's Expansion, we may assume that there is no greater
    entry than $i$ in $\mathfrak{r}'$ and in $\mathfrak{s}'$.
  \end{itemize}
  Note that all elements of $A_q(n;r,s)$
  having a factor $\mathfrak{det}_q^{(1)}$
  can be written as a linear combination of
  bideterminants of rational $(\rho,\sigma)$-bitableaux with
  $\rho\in\Lambda^+(r-k), k>0$. Thus, it suffices to show that 
  $((\mathfrak{r},\mathfrak{s})|(\mathfrak{r}',\mathfrak{s'}))$ is , 
  modulo $\mathfrak{det}_q^{(1)}$,  a linear
  combination of bideterminants 
  of 'lower content'. 
  The  summand of highest content 
  in Lemma~\ref{lem:straightening2} is that one
  for $\mathbf j=(i_1,i_2,\ldots,i_k)$, and this summand 
  is a scalar multiple (a power of $-q$, which is invertible)
  of $((\mathfrak{r},\mathfrak{s})|(\mathfrak{r}',\mathfrak{s}'))$. 
\end{proof}

The following is an immediate consequence of the preceding theorem and
Lemma~\ref{lem:bijection}.

\begin{cor}
There exists an $R$-linear map $\phi:A_q(n,r+(n-1)s)\to A_q(n;r,s)$
given on a basis by $\phi(\mathfrak{t}|\mathfrak{t}')
:=(-q)^{-c(\mathfrak{t},\mathfrak{t}')}
((\mathfrak{r},\mathfrak{s})|(\mathfrak{r}',\mathfrak{s}'))$ if the
shape $\lambda$ of $\mathfrak{t}$ satisfies $\sum_{i=1}^s\lambda_i\geq
(n-1)s$ and $(\mathfrak{r},\mathfrak{s})$, where
$(\mathfrak{r}',\mathfrak{s}')$ are the rational tableaux respectively
corresponding to $\mathfrak{t}$ and $\mathfrak{t}'$ under the
correspondence of Lemma~\ref{lem:bijection}, and
$\phi(\mathfrak{t}|\mathfrak{t}') := 0$ otherwise. We have
\[\phi\circ\iota=\mathrm{id}_{A_q(n;r,s)}\]
and thus $\pi=\iota^*$ is surjective.
\end{cor}

As noted in Section~\ref{section:submodule} we now have the main
result.

\begin{thm}[(Schur-Weyl duality for the mixed tensor space, II)]
  \label{thm:schurweyl2}
  \begin{eqnarray*}
    S_q(n;r,s)&=&\mathrm{End}_{\mathfrak{B}_{r,s}(q)}
    (V^{\otimes r}\otimes {V^*}^{\otimes s})
    =\rho_{\mathrm{mxd}}({\mathbf U})=\rho_{\mathrm{mxd}}({\mathbf U}')
  \end{eqnarray*}
Furthermore, 
$S_q(n;r,s)$ is $R$-free with a basis 
indexed by standard rational bitableau. % We call $S_q(n;r,s)$ the
%rational $q$-Schur algebra (compare \cite{dipperdoty}). 
\end{thm}
\begin{proof}
  The first assertion follows from the surjectivity of $\pi$, the
  second assertion is obtained by dualizing the basis of $A_q(n;r,s)$. 
\end{proof}       

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "mxdtensor2"
%%% End: 


==> hopf.tex <==

\section{Preliminaries}\label{section:hopf}
Let $n$ be a given positive integer.  In this section, we introduce
the quantized enveloping algebra of the general linear Lie algebra
$\mathfrak{gl}_n$ over a commutative ring $R$ with parameter $q$ and
summarize some well known results; see for example
\cite{hongkang,jantzen,lusztig}.  We will start by recalling the
definition of the quantized enveloping algebra over $\mathbb{Q}(q)$
where $q$ is an indeterminate.

Let $P^\vee$ be the free $\mathbb{Z}$-module with basis $h_1, \ldots,
h_n$ and let $\varepsilon_1, \ldots, \varepsilon_n \in {P^\vee}^*$ be
the corresponding dual basis: $\varepsilon_i$ is given by
$\varepsilon_i(h_j):=\delta_{i,j}$ for $j=1, \ldots, n$, where
$\delta$ is the usual Kronecker symbol.  For $i=1,\ldots,n-1$ let
$\alpha_i\in {P^\vee}^*$ be defined by $\alpha_i := \varepsilon_i -
\varepsilon_{i+1}$. 
\begin{defn}
  The quantum general linear algebra $U_q(\mathfrak{gl}_n)$ is the
  associative $\mathbb{Q}(q)$-algebra with $1$ 
  generated by the elements
  $e_i, f_i$ $(i=1, \ldots, n-1)$ and $q^{h}$ $(h\in P^\vee)$
  with the defining relations
  \begin{eqnarray*}
    &&q^0=1,\quad q^hq^{h'}=q^{h+h'}\\
    &&q^he_iq^{-h}=q^{\alpha_i(h)}e_i,\quad 
    q^hf_iq^{-h}=q^{-\alpha_i(h)}f_i,\\
    &&e_if_j-f_je_i=\delta_{i,j}\frac{K_i-K_i^{-1}}{q-q^{-1}},\quad
    \mbox{ where }K_i := q^{h_{i}-h_{i+1}},\\
    &&e_i^2e_j-(q+q^{-1})e_ie_je_i+e_je_i^2=0\quad\mbox{ for }|i-j|=1,\\
    &&f_i^2f_j-(q+q^{-1})f_if_jf_i+f_jf_i^2=0\quad\mbox{ for }|i-j|=1,\\
    &&e_ie_j=e_je_i,\quad f_if_j=f_jf_i\quad\mbox{ for }|i-j|>1.
  \end{eqnarray*}
\end{defn}
We note that the subalgebra generated by the $K_i, e_i, f_i$ ($i = 1,
\dots, n-1$) is isomorphic with $U_q(\mathfrak{sl}_n)$.
$U_q(\mathfrak{gl}_n)$ is a Hopf algebra with comultiplication
$\Delta$, counit $\varepsilon$ and antipode $S$ defined by
\begin{eqnarray*}
  &&\Delta(q^h)=q^h\otimes q^h,\\
  &&\Delta(e_i)=e_i\otimes K_i^{-1}+1\otimes e_i,\quad
  \Delta(f_i)=f_i\otimes 1+K_i\otimes f_i,\\
  &&\varepsilon(q^h)=1,\quad \varepsilon(e_i)=\varepsilon(f_i)=0,\\
  && S(q^h)=q^{-h},\quad S(e_i)=-e_iK_i,\quad S(f_i)=-K_i^{-1}f_i .
\end{eqnarray*}
Note that $\Delta$ and $\varepsilon$ are homomorphisms of algebras and
$S$ is an invertible anti-homomorphism of algebras.  Let
$V_{\mathbb{Q}(q)}$  be a free
$\mathbb{Q}(q)$-vector space with basis $\{v_1,\ldots,v_n\}$. We make
$V_{\mathbb{Q}(q)}$ 
into a $U_q(\mathfrak{gl}_n)$-module via
\begin{eqnarray*} 
  q^h v_j&=& 
  q^{\varepsilon_j(h)}v_j \mbox{ for }h\in P^\vee,\,j=1,\ldots,n\\
  e_iv_j&=&\left\{
    \begin{array}{ll}
      v_i&\mbox{ if }j=i+1\\
      0&\mbox{ otherwise}
    \end{array}
  \right. \hspace{3cm}
  f_iv_j=\left\{
    \begin{array}{ll}
      v_{i+1}&\mbox{ if }j=i\\
      0&\mbox{ otherwise.}
    \end{array}
  \right.
\end{eqnarray*}
We call $V_{\mathbb{Q}(q)}$ the \emph{vector representation} of
$U_q(\mathfrak{gl}_n)$.  This is also a $U_q(\mathfrak{sl}_n)$-module,
by restriction of the action.


Let $[l]_q$ (in $\mathbb{Z}[q,q^{-1}]$ resp.~in $R$) be defined by
$[l]_q:=\sum_{i=0}^{l-1}q^{2i-l+1}$, $[l]_q!:=[l]_q[l-1]_q\ldots[1]_q$
and let $e_i^{(l)}:=\frac{e_i^l}{[l]_q!}$,
$f_i^{(l)}:=\frac{f_i^l}{[l]_q!}$.  Let $\mathbf
U_{\mathbb{Z}[q,q^{-1}]}$ (resp.,
$\mathbf{U}'_{\mathbb{Z}[q,q^{-1}]}$) be the
$\mathbb{Z}[q,q^{-1}]$-subalgebra of $U_q(\mathfrak{gl}_n)$ generated
by the $q^h$ (resp., $K_i$) and the divided powers $e_i^{(l)}$ and
$f_i^{(l)}$ for $l\geq 0$. $\mathbf U_{\mathbb{Z}[q,q^{-1}]}$ is a
Hopf algebra and we have
\begin{eqnarray*} 
  \Delta(e_i^{(l)})&=&
  \sum_{k=0}^l q^{k(l-k)}e_i^{(l-k)}\otimes K_i^{k-l} e_i^{(k)}\\
  \Delta(f_i^{(l)})&=&
  \sum_{k=0}^l q^{-k(l-k)}f_i^{(l-k)}K_i^k\otimes f_i^{(k)}\\
  S(e_i^{(l)})&=& (-1)^lq^{l(l-1)}e_i^{(l)}K_i^l\\
  S(f_i^{(l)})&=& (-1)^lq^{-l(l-1)}K_i^{-l}f_i^{(l)}\\
  \varepsilon(e_i^{(l)})&=&\varepsilon(f_i^{(l)})=0.
\end{eqnarray*}
Furthermore, the $\mathbb{Z}[q,q^{-1}]$-lattice
$V_{\mathbb{Z}[q,q^{-1}]}$ in $V_{\mathbb{Q}(q)}$ generated by the
$v_i$ is invariant under the action of $\mathbf
U_{\mathbb{Z}[q,q^{-1}]}$ and of $\mathbf{U}'_{\mathbb{Z}[q,q^{-1}]}$.
Now, make the transition from $\mathbb{Z}[q,q^{-1}]$ to an arbitrary
commutative ring $R$ with $1$: Let $q\in R$ be invertible and consider
$R$ as a $\mathbb{Z}[q,q^{-1}]$-module via specializing $q\in
\mathbb{Z}[q,q^{-1}]\mapsto q\in R$. Then, let $\mathbf
U_R:=R\otimes_{\mathbb{Z}[q,q^{-1}]}\mathbf U_{\mathbb{Z}[q,q^{-1}]}$
and
$\mathbf{U}'_R:=R\otimes_{\mathbb{Z}[q,q^{-1}]}\mathbf{U}'_{\mathbb{Z}[q,q^{-1}]}$.
$\mathbf U_R$ inherits a Hopf algebra structure from $\mathbf
U_{\mathbb{Z}[q,q^{-1}]}$ and
$V_R:=R\otimes_{\mathbb{Z}[q,q^{-1}]}V_{\mathbb{Z}[q,q^{-1}]}$ is a
$\mathbf U_R$-module and by restriction also a $\mathbf{U}'_R$-module.


If no ambiguity arises, we will henceforth omit the index $R$ and
write $\mathbf{U}$, $\mathbf{U}'$ instead of $\mathbf{U}_R$,
$\mathbf{U}'_R$ and $V$ instead of $V_R$. Furthermore, we will write
$e_i^{(l)}$ as shorthand for $1\otimes e_i^{(l)}\in \mathbf{U}_R$,
similarly for the $f_i^{(l)}$, $K_i$ short for $1\otimes K_i$, and
$q^h$ short for $1\otimes q^h$.


Suppose $W, W_1$ and $W_2$ are $\mathbf U$-modules, then one can
define $\mathbf U$-module structures on $W_1\otimes W_2=W_1\otimes_R
W_2$ and $W^*=\mathrm{Hom}_R(W,R)$ using the comultiplication and the
antipode  by setting $x(w_1\otimes
w_2)=\Delta(x)(w_1\otimes w_2)$ and $(xf)(w)=f(S(x)w)$. 

\begin{defn}
  Let $r,s$ be nonnegative integers. 
  The $\mathbf U$-module $V^{\otimes r}\otimes {V^*}^{\otimes s}$ is
  \emph{called mixed tensor space}.
\end{defn}
Let $I(n,r)$ be the set of $r$-tuples with entries in $\{1,\ldots,n\}$
and let $I(n,s)$ be defined similarly.
The elements of $I(n,r)$ (and $I(n,s)$) are called \emph{multi indices}.
Note that the symmetric groups
$\mathfrak{S}_r$ and $\mathfrak{S}_s$ act on  $I(n,r)$ and  $I(n,s)$
respectively from the right
by place permutation, that is if $s_j$ is a Coxeter generator and
$\mathbf i=(i_1,i_2,\ldots )$ is a multi index, then let $\mathbf
i.s_j=(i_1,\ldots,i_{j-1},i_{j+1},i_j,i_{j+2},\ldots)$. 
Then a basis of the mixed
tensor space $V^{\otimes r}\otimes {V^*}^{\otimes s}$ can be indexed
by $I(n,r)\times I(n,s)$. For $\mathbf i=(i_1,\ldots,i_r)\in I(n,r)$ and
$\mathbf j=(j_1,\ldots,j_s)\in I(n,s)$ let
\[
v_{\mathbf i|\mathbf
  j}=v_{i_1}\otimes \ldots\otimes v_{i_r}\otimes v_{j_1}^*\otimes
\ldots\otimes v_{j_s}^*\in V^{\otimes r}\otimes {V^*}^{\otimes s}
\]
where $\{v_1^*,\ldots,v_n^*\}$ is the basis of $V^*$ dual to
$\{v_1,\ldots,v_n\}$. 
Then $\{v_{\mathbf i|\mathbf j}\mid \mathbf i\in I(n,r),\mathbf j\in
I(n,s)\}$ is a basis of $
V^{\otimes r}\otimes {V^*}^{\otimes s}$. 

We have another algebra acting on $V^{\otimes r}\otimes {V^*}^{\otimes
  s}$, namely the quantized walled Brauer algebra
$\mathfrak{B}_{r,s}^n(q)$ introduced in \cite{dipperdotystoll}. This
algebra is defined as a diagram algebra, in terms of Kauffman's
tangles. A presentation by generators and relations can be found in
\cite{dipperdotystoll}. Note that this
algebra and its action coincides with Leduc's algebra (\cite{leduc},
see the remarks in \cite{dipperdotystoll}).

Here, all we need is the action of generators given in the following
diagrams.  $\mathfrak{B}_{r,s}^n(q)$ is generated by the elements
\[
E=\raisebox{-.1cm}{\epsfbox{generators.3}},\quad
S_i=\raisebox{-.1cm}{\epsfbox{generators.1}},\quad
\hat{S}_j=\raisebox{-.1cm}{\epsfbox{generators.2}}
\]
where the non-propagating edges in $E$ connect vertices in columns
$r$, $r+1$ while the crossings in $S_i$ and $\hat{S}_j$ connect
vertices in columns $i$, $i+1$ and columns $r+j$, $r+j+1$
respectively. If $v_{\mathbf i|\mathbf j}=v\otimes v_{i_r}\otimes
v_{j_1}^*\otimes v'$, then the action of the generators on $V^{\otimes
  r}\otimes {V^*}^{\otimes s}$ is given by
\begin{eqnarray*}
  v_{\mathbf i|\mathbf j}E&=&\delta_{i_r,j_1}\sum_{s=1}^nq^{2i_r-n-1}
  v\otimes v_s\otimes v_s^*\otimes v'\\
  v_{\mathbf i|\mathbf j}S_i&=& \left\{
    \begin{array}{ll}
      q^{-1} v_{\mathbf i|\mathbf j}&\mbox{ if }i_i=i_{i+1}\\
      v_{\mathbf i.s_i|\mathbf j}&\mbox{ if }i_i<i_{i+1}\\
      v_{\mathbf i.s_i|\mathbf j}+ (q^{-1}-q)
      v_{\mathbf i|\mathbf j}&\mbox{ if }i_i> i_{i+1}
    \end{array}
  \right.\\
  v_{\mathbf i|\mathbf j}\hat{S}_j&=& \left\{
    \begin{array}{ll}
      q^{-1} v_{\mathbf i|\mathbf j}&\mbox{ if }j_j=j_{j+1}\\
      v_{\mathbf i|\mathbf j.s_j}&\mbox{ if }j_j>j_{j+1}\\
      v_{\mathbf i|\mathbf j.s_j}+ (q^{-1}-q)
      v_{\mathbf i|\mathbf j}&\mbox{ if }j_j<j_{j+1}.
    \end{array}
  \right.
\end{eqnarray*}

The action of $\mathfrak{B}_{r,s}^n(q)$ 
on $V^{\otimes r}\otimes {V^*}^{\otimes s}$ commutes with the action
of $\mathbf U$. 
\begin{thm}[\cite{dipperdotystoll}]\label{thm:Schur-Weyl_I}
  Let $\sigma: \mathfrak{B}_{r,s}^n(q)\to
  \mathrm{End}_{\mathbf U}(V^{\otimes r}\otimes
  {V^*}^{\otimes s}) $ be the representation of the quantized walled
  Brauer algebra on the mixed tensor space. 
  Then $\sigma$ is surjective, that is
  \[
  \mathrm{End}_{\mathbf U}(V^{\otimes r}\otimes
  {V^*}^{\otimes s})
  \cong 
  \mathfrak{B}_{r,s}^n(q)/_{\mathrm{ann}_{\mathfrak{B}_{r,s}^n(q)}(V^{\otimes r}\otimes
    {V^*}^{\otimes s})}.
  \] 
\end{thm}

The main result of this paper is the other half of the preceding
theorem:
\begin{thm}\label{thm:Schur-Weyl_II}
  Let $\rho_{\mathrm{mxd}}: \mathbf U\to\mathrm{End}_{ \mathfrak{B}_{r,s}^n(q) } 
  (V^{\otimes r}\otimes
  {V^*}^{\otimes s}) $ be the representation of the quantum group. 
  Then $\rho_{\mathrm{mxd}}$ is surjective, that is
  \[
  \mathrm{End}_{ \mathfrak{B}_{r,s}^n(q) }(V^{\otimes r}\otimes
  {V^*}^{\otimes s})
  \cong \mathbf U
  /_{\mathrm{ann}_{\mathbf U}(V^{\otimes r}\otimes
    {V^*}^{\otimes s})}.
  \] 
\end{thm}

Theorems~\ref{thm:Schur-Weyl_I} and \ref{thm:Schur-Weyl_II} together
state that the mixed tensor space is a $(\mathbf
U, \mathfrak{B}_{r,s}^n(q))$-bimodule with the double centralizer
property. In the literature, this is also called \emph{Schur--Weyl
  Duality}.  Theorem~\ref{thm:Schur-Weyl_II} will be proved at the end
of this paper.


For $s=0$, this is well known. $\mathfrak{B}_{m,0}^n(q)$ is the Hecke
algebra $\mathcal{H}_m$, and $V^{\otimes m}$ is the (ordinary) tensor
space. 

\begin{defn}
  If $m$ is a positive integer, let $\mathcal{H}_m$ be the associative
  $R$-algebra with one generated by elements $T_1,\ldots,T_{m-1}$ with
  respect to the relations
  \begin{align*}
    &(T_i+q)(T_i-q^{-1})=0 \mbox{ for }i=1,\ldots,m-1\\
    &T_iT_{i+1} T_i=T_{i+1} T_iT_{i+1}\mbox{ for }i=1,\ldots,m-2\\
    &T_iT_j=T_jT_i\mbox{ for } |i-j|\geq 2.
  \end{align*}
\end{defn}

  If $w\in\mathfrak{S}_m$ is an element of the symmetric group on $m$
  letters, and $w=s_{i_1}s_{i_2}\ldots s_{i_l}$ is a reduced
  expression as a product of Coxeter generators, let
  $T_w=T_{i_1}T_{i_2}\ldots T_{i_l}$. Then the set $\{T_w\mid
  w\in\mathfrak{S}_m\}$ is a basis of $\mathcal{H}_m$. 

  Note that $\mathcal{H}_m$ acts on $V^{\otimes m}$, since 
  $\mathcal{H}_m\cong \mathfrak{B}_{m,0}^n(q)$, the isomorphism given
  by $T_i\mapsto S_i$. 

\begin{thm}[\cite{dipperjamesschur,green}]
  Let $\rho_{\mathrm{ord}}:\mathbf{U} \to \mathrm{End}_R(V^{\otimes
    m})$ be the representation of $\mathbf U$ on $ V^{\otimes
    m}$. Then $\operatorname{im} \rho_{\mathrm{ord}} =
  \mathrm{End}_{\mathcal{H}_m}(V^{\otimes m})$.  This algebra is
  called the $q$-Schur algebra and denoted by $S_q(n,m)$.
\end{thm}

 We will refer to $V^{\otimes m}$ as ordinary tensor space.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "mxdtensor2"
%%% End: 


==> intro.tex <==
\section*{Introduction}
Schur-Weyl duality plays an important role in representation theory
since it connects the representations of the general linear group with
the representations of the symmetric group. The classical Schur-Weyl
duality due to Schur (\cite{schur})  states, that the actions  of the  general
linear group $G=GL_n$ and the symmetric group $\mathfrak{S}_m$ on tensor
space $V^{\otimes m}$  with $V=\mathbb{C}^n$ 
satisfy the bicentralizer property,
that is $\mathrm{End}_{\mathfrak{S_m}}(V^{\otimes m})$ is generated by
the action of $G$ and vice versa.  This duality has been generalized
to algebras which are related to the general linear group and the
symmetric group and deformations of them. 


One such generalization is the mixed tensor space  $V^{\otimes
  r}\otimes {V^*}^{\otimes s}$, which is a $\mathbb{C}G$-module. 
The centralizer algebra is known to be
the walled Brauer algebra (\cite{bchlls}) and Schur-Weyl duality holds
in this case. A $q$-deformation of these
results also exist (\cite{kosudamurakami,leduc}), but only for cases
when the centralizer algebra is semisimple. 


Let $R$ be a commutative ring with $1$ and $q\in R$ invertible. 
Let $\mathbf U$ be (an integral version of )  the quantum group over
$R$, which replaces the general linear
group in the quantized case.  
Let $S_q(n;r,s)$ be the centralizer algebra of the
$q$-deformation of the walled Brauer algebra on mixed tensor space. 
The main result of this paper states that $S_q(n;r,s)$ is the
image of the representation of
$\mathbf U$ on $V^{\otimes
  r}\otimes {V^*}^{\otimes s}$.  
We call $S_q(n;r,s)$ the \emph{rational
$q$-Schur algebra}. 
This is one half of Schur-Weyl duality for mixed tensors. 
The other part of Schur-Weyl duality on
mixed tensor space is also true  in such a general setting,
this was shown in
\cite{dipperdotystoll}. 
Furthermore, we show that the rational $q$-Schur algebra is free over
$R$ and determine a basis.


To prove Schur-Weyl duality we make use of the following fact: the mixed
tensor space $V^{\otimes r}\otimes {V^*}^{\otimes s}$ can be embedded
into a tensor
space $V^{\otimes r+(n-1)s}$. Although this embedding $\kappa$ is not a
homomorphism of $\mathbf{U}$-modules,  it is a homomorphism of
$\mathbf U'$-modules where $\mathbf U'$ is the subalgebra of $\mathbf
U$ corresponding to the special linear group. We will see that
replacing $\mathbf U$ by $\mathbf U'$ is
not significant. Associated with this embedding is an algebra
homomorphism $\pi:S_q(n,r+(n-1)s)\to S_q(n;r,s)$ where $S_q(n,r+(n-1)s)$
is the image of the representation of $\mathbf U'$ on $V^{\otimes
  r+(n-1)s}$, the \emph{(ordinary) $q$-Schur algebra}.
This  homomorphism is given by restricting to the
$\mathbf U'$-submodule $V^{\otimes r}\otimes {V^*}^{\otimes s}$ of $V^{\otimes
  r+(n-1)s}$, and the aim is to show that $\pi$ is surjective. The
algebras $S_q(n,r+(n-1)s)$ and $S_q(n;r,s)$ are the dual algebras of certain
coalgebras $ A_q(n,r+(n-1)s)$ and $A_q(n;r,s)$. We find a coalgebra map
$\iota: A_q(n;r,s)\to A_q(n,r+(n-1)s)$ such that $\iota^*=\pi$, so it
suffices to show that $\iota$ has a left inverse. We do this by giving
suitable basis for $ A_q(n,r+(n-1)s)$ and $A_q(n;r,s)$. The
description of $ A_q(n,r+(n-1)s)$ and a basis thereof is well known (see
\cite{dipperdonkin,huangzhang}). We deduce a basis for $A_q(n;r,s)$,
and thus of its dual algebra $S_q(n;r,s)$, by using determinantal
identities such as Laplace Expansion and Jacobi's Ration Theorem in a
quantized version. With these basis, a suitable left inverse for
$\iota$ can be given easily. 




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "mxdtensor2"
%%% End: 


